Characterizing Grounded Theory Approaches in Visualization

Grounded theory (GT) is a research methodology that entails a systematic workflow for theory generation grounded on emergent data. In this paper, we juxtapose GT workflows with typical workflows in visualization and visual analytics, shortly VIS, and underline the characteristics shared by these workflows. We explore the research landscape of VIS to observe where GT has been applied to generate VIS theories, explicitly as well as implicitly. We propose a "why" typology for characterizing aspects in VIS where GT can potentially play a significant role. We outline a "how" methodology for conducting GT research in VIS, which addresses the need for theoretical advancement in VIS while benefitting from other methods and techniques in VIS. We exemplify this "how" methodology by adopting GT approaches in studying the messages posted on VisGuides - an Open Discourse Forum for discussing visualization guidelines.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/OldTexFiles/Education.tex <==
% ----------------
%\begin{figure}[t]
%   \centering
%   \begin{tabular}{@{}c@{\hspace{4mm}}c@{}}
%    \includegraphics[width=\linewidth]{figures/Swansea.pdf} % &
%    \includegraphics[height=40mm,width=55mm]{Default} \\
%    Swansea
%  \end{tabular}
%  \caption{Activities of Swansea student activity at VisGuides.
%  The number in each colored cell is the number of submissions featured a particular type of visualization ($y$) on that day ($x$). The subtotals indicate the popularity of Choropleth Map and treemap.}
%  \label{fig:Swansea}
%  \vspace{-4mm}
%\end{figure}
% Reviewed by RSL on 10 Apr 2020
% ====================
\section{Data Collection in the Context of Education}
\label{sec:Teaching}

To foster data collection, VisGuides was used to support two Data Visualization courses at the University of Swansea (\swansea) during the academic years 2018/2019 and 2019/2020, and one at the University of Zurich (UZH, \zurich) during 2019/2020. The diversity of those educational environments gave us the opportunity to explore how students understand, characterize, and discuss guidelines in different scenarios.
%The motivation for this was to 
% (i) observe if VisGuides can supplement and enhance the learning experience of those who studying the topic of data visualization
%  \item To observe how visualization guidelines were used in the discussions.
%  \item \vspace*{-2mm}
%  To identify what visualization guidelines should be included in the lectures of data visualization.
% \end{itemize}
%\ben{what do you mean?:}As an important aspect of grounded theory is to look systematically for theoretical sensitivity in terms of contexts where data is collected, a hypothesis is proposed, and a conclusion emerges \cite{Strauss:1998:book}.
In addition to informing our research questions Q1 and Q2, the data we collected contributed to answering Q4.

\subsection{Context and Instructions}
Students in both courses were either in an undergraduate Bachelor of Science (BSc) or a Master of Science (MSc) computer science degree program. 

\begin{itemize}[noitemsep, leftmargin=*]

    \item \textbf{Swansea}'s students were given a visualization design challenge related to a well-known data set recording health conditions in different geographic regions.  During the course, students were instructed to use VisGuides to seek advice for their assessed visualization project by uploading work-in-progress screenshots of their class projects and \textit{``request professional help from VisGuides.org.''} Replies to posts came partly from the course instructors, partly from authors of this paper, partly from external users including researchers from the scientific visualization community, and finally also sometimes from other students. All 134 posts correspond to the first run of this exercise (questions and answers, posted between February 4 and March 13, 2019, by 64 students) and make up the focus data \swansea $~\subset$ \dataset we analyze here.

    \item \textbf{Zurich}'s exercise ran one year after Swansea's, and the students' focus was the inspection and discussion of visualization guidelines, rather than seeking advice on individual class projects. The exercise was divided into two assignments. In the first assignment, students had to look for and choose one guideline of interest from either VisGuides or any other source of visualization guidelines. Then, they had to reflect on its use and applicability. The course instructors supported this exercise with a lecture on visualization guidelines exercising critical thinking and debate. For the second assignment, students could \textit{optionally} go to VisGuides and post questions to discuss a guideline or critically answer a previous post. All 44 posts (questions and answers, posted between December 19, 2019 (launch of the assignment) and February 22, 2020 by 41 students) 
    are the focus of our data set \zurich.  % RSL: The font between zurich and swansea
    % data sets is inconsistent
\end{itemize}

% \ben{It's not clear to me which are your findings from Swansea that you learn from. If anything was important, insert that above.}
% \alex{I added some lessons learned below... last paragraph of Swansea}
%We investigated the use of visualization guidelines in two opportunities in two different universities, and with different goals in mind. The diversity of our approaches gave us the opportunity to explore how students understand, characterize, and discuss guidelines in different scenarios. We were especially interested on the benefits, advantages, disadvantages, limitations identified by the participants, as shown in the two collected datasets.
%% Swansea

% \textcolor{blue}{Possible additions: summarize how many students (out of how many) took the options, and 
% resulted in 134 posts between February 4 and March 13, 2019. Among them how many submitted an improved or 
% modified visualization instead the one posed online. Students' feedback including one example testimony. And 
% draw a conclusion on Research question (iv).}
% UZH
%The UZH assignment ran an year later, so we could apply the lessons learned from Swansea. 
%\paragraph{\textbf{Findings from the Pilot}.}First initial results from Swansea showed ....
%For Swansea, the assignment was set on February 4, 2019. A total of 64 students out of 71 participated in the VisGuides aspect of the assignment.
%From Fig. \ref{fig:Swansea}, we can observe that 41 students submitted their posts for seeking advice within the last three days of the assignment deadline (11am on March 4). 
%\alex{Here we need to focus on guidelines --> its relationships with the discussed concepts (Swansea) guidelines --> what kind of discussion is there (UZH)}
%\alex{ What the most popular Guidelines used?}
%\alex{What where the most popular concepts?}
%\alex{their relationship}
%\alex{lessons learned: how this knowledge improve the students' conceptualizatio of guidelines?}
%\alex{quotes from the questionnair}
%\paragraph{\textbf{Analysis of $D_{\text{Swansea2019}}$ and Our Findings.}}

%The majority of the posts received at least one reply. One student commented: 
%
% I asked the class if anyone used the feedback from VisGuides to improve
% their submission, however, no one responded positively to this.
%``\textit{Personally the question I myself asked did not improve much directly for my assignment, 
%however this may be [because] I had already learnt a great deal from reading all the questions and replies
%made by other students. I also learnt quite a bit about visualisation techniques I did not even 
%consider for my own assignment through VisGuides.
%At first I did not think this part would contain much substance 
% as I guessed all questions would be very similar, however, I now  think it was probably the most valuable aspect of the 
%coursework.}''
%This summarizes the typical learning experience gained by many students, in terms of \textbf{Q4} \FIX{(Did VisGuides supplement and enhance the learning experience of those who studying the topic of data visualization?).}

% \textcolor{blue}{Perhaps focusing some statistics and visualization related to (i), (ii), and (iii), and (v).}

%As shown in Fig. \ref{fig:Swansea}, 17 different chart types were featured in the students' posts. Among them, 17 students selected choropleth maps (with out without glyphs) and 20 selected treemaps as their visual designs.
%In terms of \textbf{Q4} (What visualization guidelines mentioned could be included in the lectures on data visualization?), 

\subsection{Reflections}

For all posts in \swansea{} and \zurich, we engaged in close reading. 
\paragraph{\textbf{Findings from Swansea (\swansea):}} 
The majority of the posts received at least one reply, but there was generally
not much follow-up and discussion from the students. 
% RSL: It would make sense to quantify the above statement.  How many posts
% received 1 reply?  How many 2? etc.  Express in both raw numbers and percentages.
We believe this missing engagement was due to several factors including little self-confidence to discuss topics that are new to the students, especially in discussion with visualization experts. Another factor could be the lack of training with respect to discussing design decisions, iterating over design prototypes, and scrutinize guidelines given a specific application. 
% RSL: Where do these beliefs come from?  Verbal feedback from the students?  What kind % of experience?
% We conjectured that more clear instructions and advice on critical thinking would 
% alleviate some of these problems.
However, students might also have been satisfied by the replies and did not need to discuss and iterate.
For example, one student mentioned that \textit{``Personally the question I myself asked did not improve much directly for my assignment, however this may be [because] I had already learnt a great deal from reading all the questions and replies made by other students. I also learnt quite a bit about visualisation techniques I did not even consider for my own assignment through VisGuides.''} In general that same student continued highlighting the overall benefit of VisGuides for the course work: \textit{``At first, I did not think this part would contain much substance as I guessed all questions would be very similar, however, I now think [VisGuides] was probably the most valuable aspect of the coursework.''}


From \swansea, we have identified several points where guidelines could be useful
in the context of education. For example, there were many questions about how to add temporal data to \textit{geo-spatial visualizations}.
This indicates that students could benefit from learning and discussing guidelines on this topic.
We observed similar discussions on the topics of hierarchical visualizations, treemap layout algorithms, and colors.
%
% \ben{same here. not sure this is a great finding.}
% Again students could benefit from more guidelines on  how to order variables sensibly in the hierarchy of a treemap. Although this was discussed briefly in the class, there is a clear need for dedicating more time to this topic in the future.
% Another recurring theme was the treemap layout.
% Our close-reading revealed that students generally struggled with the node placement strategy of treemap layout algorithms.
% Students could benefit from guidelines on using treemap layout algorithms.
%
As a result, the content of the data visualization course teaching content is being updated to address this need.
Also, these findings showed us the need for an introductory lecture on visualization guidelines, and the need to practice critical thinking and discussion of guidelines. 
These lessons learned were incorporated in the second session performed at UZH, \zurich.

\paragraph{\textbf{Findings from Zurich (\zurich):}} 
%For the UZH, the first assignment was set on 41 and the second assignment on 29 students out of a total of 77 participated respectively. 
%The public corpus on VisGuides that is part of this analysis,$D_{\text{UZH2020}}$, consists of 40 new posts.

%The UZH coursework, \zurich{} shows a lower participation rate than \swansea{} because the exercise was optional but a
% RSL: Again, you may want to quantify this.  Although, if the participation rate
% is too low, you may want to leave this information out altogether.
The UZH coursework featured \textbf{more diversity in terms of the selected topics, guidelines, and participation strategies:} some participants created posts about general topics.  Others answered and discussed previous posts, or followed-up on other course's posts such as how to handle outliers, inquiries about visualization techniques for multivariate analysis, discussion of color for impaired people, and ethics in visualization.

It also showed \textbf{more diversity on the way students approach the discussions of guidelines:} some participants directly named guidelines in their posts (See Section \ref{sec:VisGuides}), for example, \textit{``The Data-Ink Principle''}, \textit{``Pie Charts are bad and 3D Pie Charts are very bad''}, and \textit{``The Effects of Visual Embellishment on Comprehension and Memorability''}.
Eventually, participants engaged in longer and more detailed discussions about guidelines than in \swansea; providing references and notoriously objecting or negating previous posts. 
% Is it possible to back up the above statement with data?
% For example what was the average length of a post from
% Swansea vs Zurich?  Can you count the negations?
When asked about the utility of guidelines, students where rather positive, highlighting their ability to reassure decisions and verbalize thoughts (\textit{``[Guidelines] helped me to make more conscious decisions in design choices. Funnily enough, most of the time, I would have made the same choice based on intuition but with the help of the guidelines I was able to verbalize why I made those choices.''} (S1), \textit{``[Guidelines] help me to reflect on my visualization decisions, make them as clear as possible to users, and generally approach design more professionally.''} (S2)), as well as their ability to compress knowledge and render that knowledge accessible (\textit{``[Guidelines] help me in carefully choosing appropriate means of visualization (e.g. color or shape) in order to avoid wrong associations created by the visualization which are not present in the data itself.''}(S3)).


These findings helped us answer our research question~\textbf{Q4}.
The different views and discussions from the participants of both courses informed our data coding in Section 5 and helped us understanding how a specific set of people with different backgrounds interpret guidelines. %in this case, some of participants were completely new to the visualization community, providing a refreshing view on some topics, and sometimes well-established visualization guidelines such as the Data-Ink Ratio Principle. \ben{what refreshing look? this needs more info/proof.} 
The full list of posts, guidelines, and questionnaire results are provided as supplemental material in Appendix \ref{app:Direct}.

% In fact, this semester, we did not actually dedicate much time to this theme in the visualization class itself. We do discuss it in class, but only very briefly. The assumption was that students can figure out how to construct a data hierarchy by introducing data categories. However not all students knew how to do this.

% This is evident by looking at the questions posed on VisGuides
% in the treemaps category.
% Again, treemaps are an exceptional design, generally, in the visual
% design categories on this aspect. 
% All other visual designs incorporate an intuitive placement strategy
% and usually have clear 1- or 2-dimensional axis mappings for placement.
% 
% Treemap layout algorithms is a topic we cover in the data visualization
% class.
% However, even with the current level of topic coverage, this aspect
% still remains challenging for a significant number of students.

% \textcolor{red}{CURRENT DRAFT}
% \subsection{The Assignment and Data Source}
% The premise of the assignment is to help a research team at the 
% University of Pittsburg working on a well-known project
% called Project Tycho~\cite{burke:project}. 
% They have been collecting a massive amount of epidemiology data 
% including infectious diseases and their historical
% spread for many years now.
% The data contains information about the spatio-temporal spread
% of infectious diseases throughout history.
% The initial data collection and archive focused on the history
% of disease throughout the United States. 
% It has now expanded to include data at a global level in a standard format.
% Each data set from the project contains the following information:

%\begin{enumerate}
% \item \vspace*{-2mm}
% Condition (disease name)
% \item \vspace*{-2mm}
% DOI of data file
% \item \vspace*{-2mm}
% Number of records contained in the file
% \item \vspace*{-2mm}
% Download information
% \end{enumerate}

% There are hundreds of files that archive the years and locations
% of identified and reported disease incidence throughout history
% and across the globe.
% One of the major goals of the visualization assignment is to 
% demonstrate that visualization can be used to identify patterns,
% outliers, and gain insight into the Project Tycho data and the 
% spread of disease.

% \subsection{Instructions from the Lectures}

% The assignment refers to a hypothetical investigator called "Professor C".
% Professor C represents the average scholar in higher education that
% creates visual designs such as bar charts, line charts, and pie charts
% to observe the data.
% In this assignment, Professor C would like to obtain and convey the 
% insight contained in the Project Tycho data visually.  
% The goal is to create visualizations that maximize our understanding of the data.
% Some possible questions to investigate are:
% \begin{enumerate}
%  \item \vspace*{-2mm}
%    What does the distribution of a given disease spread look like?
%   \item \vspace*{-2mm}
%     What are the most infectious diseases?
%   \item \vspace*{-2mm}
%    Are there any interesting patterns or trends in the data?
%  \item \vspace*{-2mm}
%    Are there any outlier diseases?
%  \item \vspace*{-2mm}
%    What insight can we gain from multi-variate visualizations of the
%    data?
%  \item \vspace*{-2mm}
%    Are there any relationships between the diseases?  
%   \item \vspace*{-1mm}
%    What is the average lifespan of infectious disease spread?
% \end{enumerate}

% \textbf{Better Than Professor `C'} 
% Professor C made some attempts to visualize the data using 
% simple pie charts, bar charts, bubble charts, and line graphs. 
% He was disappointed by the results, which are not very insightful,
% nor visually informative, nor aesthetically impressive.  
% The students are asked if they can do better than Professor C.

% Students are required to select three or more appropriate visualization tools 
% for depicting the Project Tycho data.  
% They are allowed and encouraged to further abstract the data, 
% e.g., aggregating data records into groups,
% combining attributes together, 
% or adding new data, e.g., cities, geographic regions. 
% They are expected to make changes, e.g., perhaps combining some spreadsheets 
% together or creating new spreadsheets.
% Their task is to produce five different visual designs which can 
% convey meaningful and interesting insight about the data. 
% They are required to supply five unique observations about
% the data.
% The complete assignment specification is provided in an
% appendix.

% \subsection{VisGuides.org} 
% As part of the assignment, students request outside help from VisGuides. 
% Their task is to choose an image they produced and upload
% a description of the image and the image itself to VisGuides. 
% They then pose a question(s) on the site in order
% to help them complete the assignment.
% Their description also contains the DOI(s) of the data
% file(s) they used to generate the image. The DOIs let the
% users know exactly which data file(s) they used to create
% their image and enables reproducibility.

% \subsection{What happened during the assignment period?}

% Activity plot as discussed by Alex, Bob, and Min

% \subsection{What are the outcomes?}
% - Did students learn anything?\\
% - Was any visualization guideline verified.\\
% - Was any visualization guideline be considered incomplete or doubtful?\\[2mm]

% \begin{itemize}
%    \item \vspace*{-2mm}
%      What were the most frequently posted visual designs? (visual design categorization)
%    \item \vspace*{-2mm}
%      What were the most frequently posted questions? (question categorization)
%    \item \vspace*{-2mm}
%      What were the most frequently posted questions? (answer categorization)
% \end{itemize}

% Possible tables\\
%
% Possible students feedback

% Perhaps use either March 4 (coursework deadline) or March 13 (other 
% stats in the paper).

% You can also mention the number of messages after the March 4. As part 
% of the analysis, one can analyse

% - how many students left it to a very late stage, and the advice 
% received after their deadline.

% - how many students submitted reasonably early, but the advice were late.

% -------- END SWANSEA CASE STUDY ---------
%I 

==> sections/OldTexFiles/KCL-interaction.tex <==
% ====================
\section{Empirical Studies}
\label{sec:EmpiricalStudies}
%
The discussions on VisGuides often suggested that further data collection would be necessary in order for some visualization guidelines to be adequately grounded on data.
In this section, we report two empirical studies for such grounded theory processes.

% --------------------
\begin{figure}[t]
\centering
  \begin{tabular}{@{}c@{\hspace{2mm}}c@{}}
  \includegraphics[height=28.5mm]{figures/kcl-images/stimuli-ms-excel} &
  \includegraphics[height=28.5mm]{figures/kcl-images/stimuli-tableau}\\
   \small{(a) Using MS-Excel} &
  \small{(b) Using Tableau}
  \end{tabular}
  \caption{Two example screens captured by using Camtasia in an empirical study on the cost of interaction in creating bar charts.}
  \label{fig:KCL-stimuli}
  \vspace{-4mm}
\end{figure}

\begin{figure*}[t]
  \centering
  \begin{tabular}{@{}c@{\hspace{6mm}}c@{\hspace{6mm}}c@{}}
  \includegraphics[height=36mm]{figures/kcl-images/Plot-NI.pdf} &
  \includegraphics[height=36mm]{figures/kcl-images/Plot-CT.pdf} &
   \includegraphics[height=36mm]{figures/kcl-images/Plot-QA.pdf} \\
  \small{(a) Average number of interactions (NI)} &
  \small{(b) Average completion time (CT)} &
  \small{(c) Subjective judgments on easiness}
  \end{tabular}
  \caption{An empirical study on the cost of interaction. The data collected indicates that the participants' opinions about the relative easiness of use depend mainly on the task completion time, partly on the number of interactions, and in some cases, on their familiarity of the software.}
  \label{fig:KCL}
  \vspace{-4mm}
\end{figure*}
% --------------------

% -----------
% \begin{figure}[t]
%  \centering
%  \begin{tabular}{@{}c@{}}
%  \includegraphics[width=\columnwidth]{figures/kcl-images/stimuli-ms-excel}\\
%  \small{(a) Creating a plot using Microsoft Excel}\\[2mm]
%  \includegraphics[width=\columnwidth]{figures/kcl-images/stimuli-tableau}\\
%  \emph{(b) Creating a plot using Tableau}
%  \end{tabular}
%  \caption{Examples of the the stimuli used in the study.}
%  \label{fig:KCL-stimuli}
% \end{figure}

% --------------------
\subsection{A Study Inspired by ``Action without Interaction''}
\label{sec:KCL}
%
In September 2017, \textbf{east101} initiated a new thread ``Action without Interaction'' \cite{east101:2017:VisGuides} on VisGuides to discuss a guideline ``Use interaction in visualization sparsely and cautiously ...'' proposed by Gr\"{o}ller \cite{Groller:2008:Dagstuhl}. It received two replies. One (\textbf{groeller}) explained: ``interaction typically requires considerable effort and cognitive load.'' Another (\textbf{jamesscottbrown}) presented a different argument: ``... there is generally little cost (to the user) associated with adding such interactivity to a visualisation ...'' 

We wondered what would be users' opinions if they were asked. Since empirical studies are integral part of grounded theory \cite{Willig:2013:book}, we conducted a controlled experiment to collect data reflecting such ``opinions''.    
We hypothesized that \emph{the amount of interaction may influence a person's opinion as to how easy it is to use a visualization tool}.
If the same task is performed using two different tools, the tool that requires fewer interactions or less interactive time corresponds to ``using interaction'' more ``sparsely and cautiously''.

\vspace{-1mm}
\paragraph{\textbf{Study Design.}}
The study consists of four trials. For each trial, participants are required to create two bar charts to visualize a given data set. Two of the four data sets, Sa and Sb, have two columns of data and are characterized as \emph{simple data sets}. The other two data sets, Ca and Cb, have five columns of data, and are characterized as \emph{complex data sets}.
For each data, participants are first asked to perform a \emph{primary task} (T1) such that a bar chart can be produced directly based on the given data without any manipulation.
This is followed by a \emph{secondary task} (T2) that requires some simple data manipulation before a chart can be generated. The main \emph{independent variable} encodes the variation of two visualization tools used for performing these tasks. We chose to use \emph{MS-Excel} (EXL) and \emph{Tableau} (TBL).
Fig.~\ref{fig:KCL-stimuli} show two screenshots of the two visualization tools respectively.

There are 16 tool-data-task combinations, $\{$EXL, TBL$\}$ $\times$ $\{$Sa, Sb, Ca, Cb$\}$ $\times$ $\{$T1, T2$\}$. To avoid any learning effect when applying different tools to the same data set, participants were divided into two groups randomly. One group were given trials [EXL-Sa, TBL-Sb, TBL-Ca, EXL-Cb] and another were given trials [TBL-Sa, EXL-Sb, EXL-Ca, TBL-Cb]. The data sets Sa and Sb have the same numbers of rows and columns, and they were design to cause little confounding effect when they were used with different tools.
Similarly the data sets Ca and Cb were also designed to cause little confounding effect.
In other words, this allowed us to compare between the two trials in the following pairs (EXL-Sa, TBL-Sb), (TBL-Sa, EXL-Sb), (EXL-Ca, TBL-Cb), and (TBL-Ca, EXL-Cb).

The study focused on two \emph{dependent variables} -- the \emph{number of interactions} and the \emph{task completion time}. Because all participants can access a help-sheet with step-by-step instructions for each task (after 1 minute for Sa and Sb and 2 minutes for Ca and Cb), they were all able to complete the tasks. The accuracy is thus not the focus of this study.

% The \emph{apparatus} used for this study includes MS-Excel for Mac (version 16.23) and Tableau Desktop Professional Edition (version 2018.3.3). Both visualization tools were run on macOS High Sierra (version 10.13.6), iMac (Retina 5K, 2017), 3.4 GHz Intel Core i5, 32GB 2400 MHz DDR4, and Radeon Pro 570 4096 MB. Each participant was required to interact with the software using a keyboard and a mouse at the desk. All trials were recorded by both Camtasia and a camera.

\vspace{-1mm}
\paragraph{\textbf{Procedure.}} Appendix E.1 gives more detailed description about the apparatus used and the procedure for conducting the experiment.
% We arranged for the participants to take part in the experiment individually. The time taken to complete the experiment was approximately 10-25 minutes, excluding the process for obtaining consent and the pre-study explanation (5 minutes).

% Following the protocol of the university an information sheet was first given to the participant during the recruitment process. Before the pre-study explanation, a consent form was distributed for the participant to read and sign. Once the participant has agreed to take part in the study, the experimenter gave a brief explanation to the participant. The explanation included the tasks involved, the access to the help-sheet, and the sequence of the trials. The participants were informed that they could take as much time as they needed in the experiment.
%
%Following the pre-study explanation, each participant was then given a unique anonymous ID, and a demographic form to be completed for information such as gender, age group, occupation, and familiarity with the two visualization tools tested.
For each participant, the experiment consisted of four trials, either [EXL-Sa, TBL-Sb, TBL-Ca, EXL-Cb] or [TBL-Sa, EXL-Sb, EXL-Ca, TBL-Cb]. In each trial, the data set was pre-loaded onto the visualization tools. Participants were given written specification of the tasks together with examples of the bar charts to be created. After an initial attempt of 1 minute for tasks associated with data sets Sa and Sb and 2 minutes for tasks with data sets Ca and Cb, participants were allowed to make use of a help-sheet to complete the task. At the end of the second trial, participants ware presented with two questions (for T1 and T2 with Sa and Sb) about the easiness of using the two visualization tools. They are asked to rank the relative easiness using the Likert scale. Similarly at the end of the fourth trial, participants were presented with three questions (for T1 and T2 with Ca and Cb, and for the overall impression).

\vspace{-1mm}
\paragraph{\textbf{Participants.}}
A total of 20 participants (12 females, 8 males) took part in this experiment in return for a \pounds5 Amazon voucher. Participants were recruited from King's College London. They belong to both the student and working communities and are from a number of disciplines, including history, psychology, business, politics, mathematics, law, and computer science. 17 participants were in the 20-29 age group and 3 were in the 18-19 age group. In rating their experience in using MS-Excel, 3 rated ``beginner'', 16 rated ``intermediate'', and 1 rated ``advanced''. In the rating of their experience in using Tableau, 18 rated ``never'', 1 rated ``beginner'', and 1 rated ``intermediate''.

% \begin{figure}[t!]
%  \centering
%  \begin{tabular}{@{}c@{}}
%  \includegraphics[width=\columnwidth]{figures/kcl-images/avg-steps}\\
%  (a) Average number of steps\\
%  \includegraphics[width=\columnwidth]{figures/kcl-images/avg-completion-time}\\
%  (b) Average completion time
%  \end{tabular}
%  \caption{Summary of the performance results of each data sets with the associated software applications.}
%  \label{fig:KCL-summary-results}
% \end{figure}

% \begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/kcl-images/subjective-questionnaire}
%    \caption{Results of the subjective questionnaire. Q1: For preparing the first plot (without sorting), which software is easier to use?. Q2: For preparing the second plot (with sorting), which software is easier to use?. Q3: For preparing the first plot (comparing 4 products), which software is easier to use?. Q4: For preparing the second plot (growth per product), which software is easier to use?. Q5: For all four data sets, overall which software is easier to use?}
%     \label{fig:KCL-subjective-results}
% \end{figure}

% \begin{table}[t]
% \caption{The ANOVA results to accompany Figure \ref{fig:KCL-summary-results}(a,b).}
% \label{tab:KCL-ANOVA}
% \centering
% \begin{tabular}{@{}r@{\hspace{2mm}}c@{}}
% \small{\textbf{Data Type}} & \small{\textbf{MS-Excel v Tableau}}\\
% \hline
% \small{Simple - primary (steps)} & 0.85\\
% \small{Simple - primary (CT)} & 0.0056\\
% \hline
% \small{Simple - secondary (steps)} & 0.069\\
% \small{Simple - secondary (CT)} & 0.41\\
% \hline
% \small{Complex - primary (steps)} & 0.00044\\
% \small{Complex - primary (CT)} & 0.0000027\\
% \hline
% \small{Complex - secondary (steps)} & 0.02427\\
% \small{Complex - secondary (CT)} & 0.0041\\
% \hline
% \end{tabular}
% \end{table}

\vspace{-1mm}
\paragraph{\textbf{Results and Discussion.}}
From the collected data, we first extracted the number of interactions (NI) and the task completion time (CT) per participant, trial and task, yielding $20 \times 4 \times 2$ pairs of (NI, CT). After confirming that there were no confounding effects between Sa and Sb and between Ca and Cb, we created a combined group EXL-S-T1 by merging the data of EXL-Sa-T1 and EXL-Sb-T1, and the other seven combined groups in a similar manner.
We therefore compute eight pairs of average (NI, CT) for EXL-S-T1, TBL-S-T1, EXL-S-T2, TBL-S-T2, EXL-C-T1, TBL-C-T1, EXL-C-T2, and TBL-C-T2.

Figs.~\ref{fig:KCL}(a,b) show the eight average values of NI and eight average values of CT respectively.
Fig.~\ref{fig:KCL}(c) summarizes the participants' answers to the five questions. Each bar indicates the number of participants who rated the easiness in one of the five Likert points.
The ANOVA results indicate that most pairwise comparisons in Figs.~\ref{fig:KCL}(a,b) are significant, except the first two NI averages in Fig.~\ref{fig:KCL}(a) for EXL-S-T1 vs. TBL-S-T1. The initial analysis also cast a doubt on the statistical significance of the pairwise comparison EXL-S-T2 vs. TBL-S-T2 in terms of both NI and CT. A close examination of the data revealed a single outlier because a participant resisted to consult the help-sheet after many failed attempts in this particular trial. After removing the data of this outlier, the ANOVA indicated convincing statistical significance. 
From these statistics, we can make the following observations:
% Tableau performed better in number of steps comparison to MS-Excel although it is statistically insignificant. Looking through the raw data, we noticed that this is because of a performance of a participant with an unusual high number of steps to complete this task. When we removed this participant data from the analysis for simple and secondary task, the result showed that Tableau performed significantly better than Microsoft Excel ($p<0.0045$). For the completion time in the simple and secondary data set, both Microsoft Excel and Tableau performs almost equally the same.
%
\begin{itemize}
  \vspace{-1mm}%
  \item For the simple data sets (Sa and Sb), MS-Excel and Tableau incurred similar numbers of interactions for performing the primary task (T1), while MS-Excel required less time than Tableau (which could be influenced by familiarity). The participants' opinions on the relative easiness are in favor of Excel.
  \vspace{-1mm}%
  \item For the simple data sets (Sa and Sb), Tableau incurred fewer interactions and less task completion time for performing the secondary task (T2). The participants' opinions are in favor of Tableau.
  \vspace{-1mm}
  \item For the complex data sets (Ca and Cb), MS-Excel incurred noticeably fewer interactions and shorter task completion time for performing the primary task (T1). The participants' opinions are overwhelmingly in favor of Excel.
  \vspace{-1mm}
  \item For the complex data sets (Ca and Cb), Tableau incurred fewer interactions and less task completion time for performing the secondary task (T2). However, the participants' opinions are marginally in favor of Excel. This inconsistency may be caused by the participants' familiarity of the software or their experience of the proceeding task. 
  \vspace{-1mm}
  \item The participants' overall impression is in favor of MS-Excel, which is consistent with the overall NI and CT measures collected.
\end{itemize}
Based on the above observations, we conclude that participants' opinions on the relative easiness depend mainly on the task completion time, and to some extent also on the number of interactions. In some cases, the familiarity of the software may modify the direct correlations among NI, CT, and subjective judgment.
In term of \textbf{Q6} in Section \ref{sec:Introduction}, while this study provides a new collection of data on which the guideline ``Use interaction in visualization sparsely and cautiously ...'' \cite{Groller:2008:Dagstuhl} can be grounded, we recognize that more grounded theory activities are necessary in order to achieve theoretical saturation.

==> sections/OldTexFiles/KCL-interaction_2020.tex <==
% ====================
\section{Empirical Studies}

\begin{figure*}[t]
  \centering
  \begin{tabular}{@{}c@{\hspace{6mm}}c@{\hspace{6mm}}c@{}}
  \includegraphics[height=36mm]{figures/kcl-images/Plot-NI.pdf} &
  \includegraphics[height=36mm]{figures/kcl-images/Plot-CT.pdf} &
   \includegraphics[height=36mm]{figures/kcl-images/Plot-QA.pdf} \\
  \small{(a) Average number of interactions (NI)} &
  \small{(b) Average completion time (CT)} &
  \small{(c) Subjective judgments on easiness}
  \end{tabular}
  \caption{An empirical study on the cost of interaction. The data collected indicates that the participants' opinions about the relative easiness of use depend mainly on the task completion time, partly on the number of interactions, and in some cases, on their familiarity of the software.}
  \label{fig:KCL}
  %\vspace{-4mm}
\end{figure*}
\label{sec:EmpiricalStudies}
%Reading and replying to posts on VisGuides made us spotting discussions that lacked empirical evidence for both supporting advice and informing a discussion grounded in data (Fig. 2-D3). \ben{As traditionally, empirical studies are not part of grounded theory \cite{Willig:2013:book}, we \textit{amend} the traditional GT by conducting controlled experiments to collect data reflecting  ``\textit{opinions}'' stated in the forum.} 
%In fact, many statements in the forum, relating to topics such as color design for color impaired people~\cite{colorblinded:2020:VisGuides}, data ethics in visualization~\cite{dataethics:2020:VisGuides}, and gamification in visual design~\cite{gamification:2020:VisGuides}, can serve to deduce hypotheses that can then be tested empirically in controlled user studies. \ben{Besides their ability to support or reject hypotheses, we want to show how controlled studies could provide additional data for grounding guidelines, make for specific cases, inform new hypotheses and guidelines, and add to theoretical saturation of guidelines through goal-driven, controlled, and rigorous data collection. This section reports on two controlled user studies, informed by discussions in our forum.}

The discussions on VisGuides often suggested that further data collection would be necessary in order for some visualization guidelines to be adequately grounded on data (Fig. 2-D3).
Researchers have argued for the extension of the traditional GT to include controlled empirical studies in order to evaluate and validate hypotheses \cite{Corbin:QS:1990, Weingand:IFLA:1993, Henwood:APA:2003, Badreddin:USER:2012}.
In the field of visualization, such extension and close linkage makes sense as they enable us to deduce a hypothesis and empirically test the hypothesis. In this section, we report two empirical studies for such grounded theory processes.

% --------------------
% \begin{figure}[t]
% \centering
%   \begin{tabular}{@{}c@{\hspace{2mm}}c@{}}
%   \includegraphics[height=28.5mm]{figures/kcl-images/stimuli-ms-excel} &
%   \includegraphics[height=28.5mm]{figures/kcl-images/stimuli-tableau}\\
%   \small{(a) Using MS-Excel} &
%   \small{(b) Using Tableau}
%   \end{tabular}
%   \caption{Two example screens captured by using Camtasia in an empirical study on the cost of interaction in creating bar charts.}
%   \label{fig:KCL-stimuli}
%   \vspace{-4mm}
% \end{figure}


% --------------------

% -----------
% \begin{figure}[t]
%  \centering
%  \begin{tabular}{@{}c@{}}
%  \includegraphics[width=\columnwidth]{figures/kcl-images/stimuli-ms-excel}\\
%  \small{(a) Creating a plot using Microsoft Excel}\\[2mm]
%  \includegraphics[width=\columnwidth]{figures/kcl-images/stimuli-tableau}\\
%  \emph{(b) Creating a plot using Tableau}
%  \end{tabular}
%  \caption{Examples of the the stimuli used in the study.}
%  \label{fig:KCL-stimuli}
% \end{figure}

% --------------------
\subsection{Study I: \textit{Action without Interaction}}
\label{sec:KCL}
%

\newcommand{\hi}{\textsc{H1}}

In September 2017, forum user \texttt{east101} initiated a thread \textit{Action without Interaction} \cite{east101:2017:VisGuides} on VisGuides to discuss a guideline \textit{``Use interaction in visualization sparsely and cautiously ...''} that had been stated by Eduard Gr\"{o}ller in a Dagstuhl seminar report abstract~\cite{Groller:2008:Dagstuhl}. In the forum, user \texttt{groeller} clarified that \textit{``interaction typically requires considerable effort and cognitive load.''}. User \texttt{jamesscottbrown} later presented a contrasting argument: \textit{``... there is generally little cost (to the user) associated with adding such interactivity to a visualisation ...'}'. From this discussion, we deduced the following hypothesis which we can test in a controlled user study: \textbf{\hi: The amount of interaction necessary to achieve a task negatively correlates with a person's perception as to how easy a visualization tool is to use.} In other words, if the same task would be performed using two different tools, the tool that requires fewer interactions or less time to interact would reduce effort and cognitive load.

% \paragraph{\textbf{Conditions and context}}
%If the same task is performed using two different tools, the tool that requires fewer interactions or less interactive time corresponds to "using interaction" more "sparsely and cautiously".
%% AD: There is a lot of literature in this topic, that could also support our empirical studies... especially from HCI.
% Among the conditions that we considered are:
% \begin{enumerate}
%     \item similarity among the tools. We chose to use \emph{MS-Excel} (EXL) and \emph{Tableau} (TBL).\alex{why? is it because MS-Excel is pervasive and Tableau is a well-known tool in our community?. How does the selection of the tools reflect the hypothesis we would like to test: "the amount of interaction may influence a person's opinion as to how easy it is to use a visualization tool"??}
% Fig.~\ref{fig:KCL-stimuli} shows two screenshots of the two visualization tools respectively.
%     \item familiarity of the users to the tool. 
%     \item tasks to be performed.
% \end{enumerate} 
% \vspace{-1mm}

\newcommand{\texcel}{\textsc{MS Excel}}
\newcommand{\ttableau}{\textsc{Tableau}}

\paragraph{\textbf{Study Design:}}
%% Setup
This study compared two tools, \texcel{} and \ttableau, as both provide different ways and interactions to perform a specific visualization task. Our study consisted of four trials in which participants were required to create two bar charts to visualize a given data set. \textbf{Data sets:} Two of the four data sets, \texttt{D1} and  \texttt{D2}, have two columns of data and are characterized as \emph{simple}. The other two data sets, \texttt{D3} and \texttt{D4}, have five data columns and are considered \emph{complex}.
\textbf{Tasks:} For each data set \texttt{D1-D4}, participants first had to perform task \texttt{T1} to produce a bar chart directly from the data without any manipulation. \texttt{T1} was followed by \texttt{T2} that required some simple data manipulation before a chart would be generated. The  \textbf{independent variable} was the variation of two visualization tools used for performing these tasks. 
\textbf{Dependent variables:} During the study, we measured \emph{number of interactions}, \emph{task completion time} and after each task, participants were asked to rank task \textit{easiness} using a Likert scale. A total of 20 participants (12 females, 8 males) took part in the study. The full study design and protocol is found in Appendix E.1.


% R3-2: - the two follow-up studies had some serious flaws and weren’t really addressing the research questions posed. E.g., the first study seemed to explore interactivity in the creation of a chart, when the interactive component of the original guideline was referring to the interactivity of the visualization itself
%% Conditions

%% R2-6: Section 7: These studies are the weakest part of the paper: The experimental "manipulations" do not really allow to evaluate the design guidelines as postulated. You did NOT manipulate interactivity in 7.1, but compared two different tools. Why do you think Tableau and Excel systematically differ in interactivity? The most profound difference is students familiarity with it (as is discussed also in the paper). In the study in 7.2 I would have understood the guideline differently and would have tried to replicate the data in "real world" style, e.g. mountains with snow on top instead of neutral data visualizations. When you add only a visual environment, you increase the visual information, so you would need a control condition with the same amaount of (more neutral / abstract) information in the environment.

%\alex{This can go to the appendix.}
%There are 16 tool-data-task combinations, $\{$EXL, TBL$\}$ $\times$ $\{$Sa, Sb, Ca, Cb$\}$ $\times$ $\{$T1, T2$\}$. To avoid any learning effect when applying different tools to the same data set, participants were divided into two groups randomly. One group were given trials [EXL-Sa, TBL-Sb, TBL-Ca, EXL-Cb] and another were given trials [TBL-Sa, EXL-Sb, EXL-Ca, TBL-Cb]. The data sets Sa and Sb have the same numbers of rows and columns, and they were design to cause little confounding effect when they were used with different tools.
%Similarly the data sets, Ca and Cb were also designed to cause little confounding effect.
%In other words, this allowed us to compare between the two trials in the following pairs (EXL-Sa, TBL-Sb), (TBL-Sa, EXL-Sb), (EXL-Ca, TBL-Cb), and (TBL-Ca, EXL-Cb).


% \begin{figure}[t!]
%  \centering
%  \begin{tabular}{@{}c@{}}
%  \includegraphics[width=\columnwidth]{figures/kcl-images/avg-steps}\\
%  (a) Average number of steps\\
%  \includegraphics[width=\columnwidth]{figures/kcl-images/avg-completion-time}\\
%  (b) Average completion time
%  \end{tabular}
%  \caption{Summary of the performance results of each data sets with the associated software applications.}
%  \label{fig:KCL-summary-results}
% \end{figure}

% \begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/kcl-images/subjective-questionnaire}
%    \caption{Results of the subjective questionnaire. Q1: For preparing the first plot (without sorting), which software is easier to use?. Q2: For preparing the second plot (with sorting), which software is easier to use?. Q3: For preparing the first plot (comparing 4 products), which software is easier to use?. Q4: For preparing the second plot (growth per product), which software is easier to use?. Q5: For all four data sets, overall which software is easier to use?}
%     \label{fig:KCL-subjective-results}
% \end{figure}

% \begin{table}[t]
% \caption{The ANOVA results to accompany Figure \ref{fig:KCL-summary-results}(a,b).}
% \label{tab:KCL-ANOVA}
% \centering
% \begin{tabular}{@{}r@{\hspace{2mm}}c@{}}
% \small{\textbf{Data Type}} & \small{\textbf{MS-Excel v Tableau}}\\
% \hline
% \small{Simple - primary (steps)} & 0.85\\
% \small{Simple - primary (CT)} & 0.0056\\
% \hline
% \small{Simple - secondary (steps)} & 0.069\\
% \small{Simple - secondary (CT)} & 0.41\\
% \hline
% \small{Complex - primary (steps)} & 0.00044\\
% \small{Complex - primary (CT)} & 0.0000027\\
% \hline
% \small{Complex - secondary (steps)} & 0.02427\\
% \small{Complex - secondary (CT)} & 0.0041\\
% \hline
% \end{tabular}
% \end{table}

\paragraph{\textbf{Results:}}
%From the collected data, we first extracted the number of interactions (NI) and the task completion time (CT) per participant, trial and task, yielding $20 \times 4 \times 2$ pairs of (NI, CT). After confirming that there were no confounding effects between Sa and Sb and between Ca and Cb, we created a combined group EXL-S-T1 by merging the data of EXL-Sa-T1 and EXL-Sb-T1, and the other seven combined groups in a similar manner.
%We therefore compute eight pairs of average (NI, CT) for EXL-S-T1, TBL-S-T1, EXL-S-T2, TBL-S-T2, EXL-C-T1, TBL-C-T1, EXL-C-T2, and TBL-C-T2.

Figs.~\ref{fig:KCL}(a,b) shows the \textit{number of interactions} across techniques (\texcel{} and \ttableau), tasks (\texttt{T1-T2}) and data sets (simple: \texttt{D1}, \texttt{D2}; complex: \texttt{D3}, \texttt{D4}) while Fig.~\ref{fig:KCL}(c) summarizes participants' subjective ratings for how easy each task was for different levels of data difficulties (S, C) and tasks (\texttt{T1-T4}). 
%
%The ANOVA results indicate that most pairwise comparisons in Figs.~\ref{fig:KCL}(a,b) are significant, except the first two NI averages in Fig.~\ref{fig:KCL}(a) for EXL-S-T1 vs. TBL-S-T1. The initial analysis also cast a doubt on the statistical significance of the pairwise comparison EXL-S-T2 vs. TBL-S-T2 in terms of both NI and CT. A close examination of the data revealed a single outlier because a participant resisted to consult the help-sheet after many failed attempts in this particular trial. After removing the data of this outlier, the ANOVA indicated convincing statistical significance. 
%From these statistics, we can make the following observations:
% Tableau performed better in number of steps comparison to MS-Excel although it is statistically insignificant. Looking through the raw data, we noticed that this is because of a performance of a participant with an unusual high number of steps to complete this task. When we removed this participant data from the analysis for simple and secondary task, the result showed that Tableau performed significantly better than Microsoft Excel ($p<0.0045$). For the completion time in the simple and secondary data set, both Microsoft Excel and Tableau performs almost equally the same.
%
%\begin{itemize}
%  \vspace{-1mm}%
%  \item For the simple data sets (Sa and Sb), MS-Excel and Tableau incurred similar numbers of interactions for performing the primary task (T1), while MS-Excel required less time than Tableau (which could be influenced by familiarity). The participants' opinions on the relative easiness are in favor of Excel.
%  \vspace{-1mm}%
%  \item For the simple data sets (Sa and Sb), Tableau incurred fewer interactions and less task completion time for performing the secondary task (T2). The participants' opinions are in favor of Tableau.
%  \vspace{-1mm}
%  \item For the complex data sets (Ca and Cb), MS-Excel incurred noticeably fewer interactions and shorter task completion time for performing the primary task (T1). The participants' opinions are overwhelmingly in favor of Excel.
%  \vspace{-1mm}
%  \item For the complex data sets (Ca and Cb), Tableau incurred fewer interactions and less task completion time for performing the secondary task (T2). However, the participants' opinions are marginally in favor of Excel. This inconsistency may be caused by the participants' familiarity of the software or their experience of the proceeding task. 
%  \vspace{-1mm}
%  \item The participants' overall impression is in favor of MS-Excel, which is consistent with the overall NI and CT measures collected.
%\end{itemize}
Based on the results shown in Fig.~\ref{fig:KCL}, we conclude that participants' opinions on the relative easiness depend mainly on \textit{task completion time}, and only to some extent also on \textit{number of interactions}. In some cases, the familiarity of the software may modify the direct correlations among \textit{number of interactions}, \textit{task completion time}, and subjective judgment. Our results show that participants' perception of \textit{easiness} seem to depend more on the time spend with a tool than the number of interactions. To some extend these results contradict \hi{} and thus some part of the guideline posed in the forum. 
%That is, depending on additional evidence through more empirical studies, there are at least three options how our results contest the initial guideline: (a) the initial guidelines would need to be \textit{rejected}, (b) the initial guideline has several cases where it is not valid and can be systematically \textit{amended} (e.g., ``.. except for very simple tasks and expert users ''), or (c) our study found is part of a (possible) set of cases which do not allow to make any structured and generic amendments to the initial guideline. 
\paragraph{\textbf{Implications:}}
In the context of this study and \hi{}, our results could account for an \textit{exception} to an otherwise \textit{acceptable} guideline, e.g., depending on our setup, participants, tasks, or tool choices. Additional evidence through more empirical studies, is needed to find out if: 
\textit{(a)} there are other cases where the initial guideline is not valid and the guideline has to be systematically \textit{amended} to exclude individual cases (e.g., \textit{``.. except for very simple tasks and expert users ''}), or 
\textit{(b)} our study is part of a (possible) set of cases which do not allow any structured and generic amendments to the initial guideline, i.e., there exist a list of unrelated exceptions that cannot be traced back to a common factor, or 
\textit{(c)} the guideline has to be rejected for most cases based on an extensive and careful set of empirical studies. Of course, more empirical data is required to advance the discussion for this specific guideline, driven by the same hypothesis as ours as well as others deduced from explicit guideline statements, arguments, cases and examples, and entire discussion threads.
%\alex{I reformulated this sentence a bit, we are way too far to "reject" a guideline, and that could also be read a bit harsh... IMO}
%In terms of \textbf{Q6} in Section \ref{sec:Introduction}, while this study provides a new collection of data on which the guideline ``Use interaction in visualization sparsely and cautiously ...'' \cite{Groller:2008:Dagstuhl} can be grounded, we recognize that more grounded theory activities are necessary in order to achieve theoretical saturation.

==> sections/OldTexFiles/Konstanz-VR.tex <==
% R1-21: The analysis in this section is questionable (removing outlier), the premise is also not clearly derived from the data and involving participants who are more familiar with one condition than the other undermines all efforts to compare. Consequently the study does little to help us determine whether or not we are to “Use interaction in visualization sparsely and cautiously”. I feel quite strongly that it would be wrong to publish the results of this study (S7.1). I'd say the same about the "Don’t Replicate the Real World" study as well (S7.2) - it doesn't help us assess the guideline very effectively or convincingly. I would question the use of a completion time metric when participants who are new to a research setting are informed that they are "allowed to take as much time as they wish to complete the task". There is more to see in one condition and participants may wish to spend time seeing it. Results are presented in a hurry with no  detail about assumptions or concepts (what is a layer movement?) Are the error bars shown in Fig 12 95% confidence intervals? They should be labeled. They are hard to believe. The results are not clear from this. Reporting varying p-values post-hoc is not good practice. Working with point and interval estimates (e.g. sample means and confidence intervals) may be more effective and convincing. Also, see Error Bars Considered Harmful (10.1109/TVCG.2014.2346298)
% R3-6:   Lastly, the paper suffers a bit from trying to shoehorn in two informal studies that are mostly unconnected to the GT study run on the website. The first study comparing Excel to Tableau seems to be a usability study of chart creation, but what does that have to do with InfoVis interactivity? Typically, that kind of guideline is referring to the ability to interact with the _data_ (e.g., to brush over the bars to see labels, to drag bars to re-order, etc.). The second study is a bit better, but focuses on VR environments, which in the GT study appear to only be relevant to 0.8% of the posts. It is also unclear whether what’s being tested is a genuine interpretation of the guideline proposed by Elmqvist, as the purpose of the “real-world” in VR is to facilitate navigation and provide awareness of surroundings, which is not the same as creating a fake office-like environment in a dataset rendered on a desktop machine. I would recommend removing these two studies from the paper entirely.

% --------------------
\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/Method21Konstanz/scenarios.png}
  \centering
  \caption{Left: Plain condition, Right: Office condition. In each condition, participants performed an comparative visual exploration task. }
 \label{fig:Konstanz-stimuli}
 %\vspace{-4mm}
\end{figure}
% --------------------

%% AD: move to the appendix
%\begin{figure*}[t]
%  \centering
%  \begin{tabular}{@{}c@{\hspace{2mm}}c@{\hspace{4mm}}c@{\hspace{2mm}}c@{}}
%    \includegraphics[height=44mm]{figures/Method21Konstanz/Plot-P1P2-Plain.pdf} &
%    \includegraphics[height=44mm]{figures/Method21Konstanz/Plot-P1P2-Office.pdf} &
%    \includegraphics[height=44mm]{figures/Method21Konstanz/Plot-MvTm-Plain.pdf} &
%    \includegraphics[height=44mm]{figures/Method21Konstanz/Plot-MvTm-Office.pdf} \\
%    \small{(a) Plain: distances to Peak 1 and Peak 2} &
%    \small{(b) Office: distances to Peak 1 and Peak 2} &
%    \small{(c) Plain: \# moves vs. completion time} &
%    \small{(d) Office: \# moves vs. completion time}
%  \end{tabular}
%  \caption{Four scatter plots show the collected measurements from the 180 trials in the plain 3D environment, and the 180 trials in the office VE. The four measurements are the distance from the pointer location to Peak 1 (i.e., the correct peak in surface 1), the distance to Peak 2, the number of layer movements, and the task completion time.}
%  \label{fig:Konstanz-ScatterPlots}
%  \vspace{-4mm}
%\end{figure*}
%
% ==========
\subsection{Study II: \textit{Don't Replicate the Real World}}
\label{sec:Konstanz}

\newcommand{\hii}{\textsc{H2}}

In May 2018, user \texttt{matthias.kraus} initiated a discussion thread ``\textit{(Don't / Do) Replicate the Real World in VR?}''~\cite{kraus:2018:VisGuides}. In this thread, the user asked about the transferability of a guideline that had been formulated as a ``rule'' by Niklas Elmqvist in his blog~\cite{Elmqvist:2017:blog}---\textit{``Rule \#7: Don't Replicate the Real World''}. \texttt{Matthias.kraus} was asking if the guideline would still hold when applied to virtual reality (VR), arguing that \textit{``familiar surroundings [would] lower the learning curve [for visual analysis environments]''}. The thread received a fair amount of discussion, among others, a comment by Nilkas Elmqvist (user \texttt{elm}), confirming that his guideline was meant to include VR. 

The discussion motivated us to formulate and test a hypothesis: \textbf{\hii: 
realistic surroundings in virtual reality environments distract people while completing a task, which leads to longer task completion times and increased interaction effort.} %a realistic background encourages people to spend more time in an virtual environment, more time on the task and consequently more accurate results.} 
%Rather than testing the initial and comprehensive guideline itself, which also includes user interaction and interfaces in general, our \hii{} is inspired by the forum discussion on the generalizability of the guideline, focusing on a basic aspect of replication which is easy to control in a user study. 
Since the initial guideline is expressed in a very general way that covers a range of conditions, variables, and contexts, we focused our study on a specific \textit{case} of replication. Rather than testing the initial guideline in its entire extent, which would include the realistic replication of user interaction and interfaces, \hii{} is inspired by the forum discussion on the generalizability of the guideline and focuses on the basic aspect of replication in VR environments. To that end, our study focuses on how realistic the environment is, not the visualization itself.

%\EDIT{Since the initial guideline is expressed in a very general way that covers various conditions, variables, and contexts, in our study, we focused on a specific \textit{case} of replication: (i) a realistic environment 
%and (ii) evaluating only task completion time, amount of user interactions, and task accuracy. %As analysis context (iii), we deployed a visualization setup with 3D heatmaps \ben{these are heatmaps?} for a comparative analysis task, and basic interaction with VR controllers.

% \paragraph{\textbf{Hypothesis, conditions, and context.}}
%Following the discussions, the PhD student who initiated the thread decided to conduct a controlled experiment to collect more data in order evaluate the guideline in the context of his hypothesis. This became part of the research question \textbf{Q6} in Section \ref{sec:Introduction}.
%If having a visually-realistic virtual environment (VE) does not impact on tasks of visual exploration negatively, one would have to reconsider this guideline. 

\newcommand{\plain}{\texttt{Plain}}
\newcommand{\real}{\texttt{Real}}

\paragraph{\textbf{Study Design:}} The study tested two conditions of an analytic setup in an immersive VR environment (Fig.~\ref{fig:Konstanz-stimuli}): one environment imitated an office space (\real), the other one did not feature any background (\plain). In each environment, participants were asked to perform two tasks to find \emph{common peaks} (\textbf{T1}) in two bivariate surfaces and to select \textit{two highest peaks} (\textbf{T2}) among all common peaks. Participants could use simple controls to move both surfaces into each other. During the study, we measured \textbf{dependent variables} \textit{task completion time}, the \textit{number of layer movements} made during each trial, and \textit{precision}. Participants had as much time as they wished to complete task. 12 participants (2 females) participated in our study. More detail about this study setup and apparatus can be found in Appendix E.2.


\begin{figure}[t]
    \centering
    \includegraphics[width=70mm]{figures/Method21Konstanz/Plot-Barcharts.pdf}
    \caption{Comparing the average accuracy ($100\%=1$), the average task completion time, and the average percentage of trials with layer movement ($20\%=0.2$) in the plain 3D environment and the office VE.}
    \label{fig:Konstanz-Barcharts}
    %\vspace{-4mm}
\end{figure}

% As shown in Fig. \ref{fig:teaser}(c), the main \emph{apparatus} used is a HTC Vive Pro VR headset (GTX1080Ti, SSD, and 16GB RAM). The experiment was carried out in a $7m \times 7m$ physical laboratory, where each participant performed their tasks in the middle of the room while the experimenter sat a few meters away by the computer that controls the virtual environment.
% As shown in Fig. \ref{fig:Konstanz-stimuli}, the plain 3D environment contains only a cube on a plane. The top of the cube is the reference plane for the two height fields. The  visually-realistic VE has a $1m^2$ table in the middle of an office environment (walkable area: $5m \times 5m$). The top of the table is the reference plane for the two height fields. 
% The virtual office itself is of $7m \times 20m$ including all spaces for the background objects.

%\paragraph{Hypothesis}
% Participants perform worse when a realistic environment is provided. This could be due to distraction and decreased readability of heightmaps for comparison\\

% \paragraph{\textbf{Procedure.}}
% Fig.~\ref{fig:teaser}(c) shows the main \emph{apparatus} used  in this experiment. Appendix E.2 describes the apparatus and the procedure in detail.
%All participants first attended an introduction session. With aid of presentation slides, we described concept of height fields and their typical visual representations, such as heat-maps and 3D surfaces (height-maps). Using examples of real world data (e.g., geographical maps with bi-variate distributions of crime rates and arrest rates, participants became accustomed to the visual observation of height fields, the interpretation of peaks and valleys, and the recognition of similar geometric features between two height fields. They were made aware of the tasks to be performed during the experiment, i.e., identifying common peaks.
%
%The participants would then undergo a training session for working with the VR equipment, including interactive controls for navigation and command selection. Each participant was asked to complete 10 interactive tasks, and was required to repeat the exercise until all tasks were completed without errors.
%

% 1) Introduction / teaching by use of slides\\
% After participants were welcomed, we started with a teaching session on heatmaps and heightmaps, introducing them to the basic interpretation of such visualizations. This contained which variables are encoded how (position, color) and how to extract information from the visualization (e.g., height goes from value 0 to 10 - if surface is on 40\% height that means its value is 4). We used an real world example of distributions for explanation of heightmaps - geo referenced heightmaps describing crime rates (i.e., where in a city crimes were reported; quantity per position) and arrest rates (i.e., where in a city people were arrested for crimes; quantity per position). Using this example we could explain the term of correlation (where both distributions have a peak) and explain the focus on high levels of ''correlation`` - i.e., for us only interesting if correlation is on high level (high peaks at same position)\\
% 2) in VR: Training phase, interactive walk-through through task, interaction possibilities and procedure. Repeated until all example scenarios (10) were completed without error. \\
% 3) block1: With/Without office 15 trials\\
% 4) block2: with/without office 15 trials\\
% 3 and 4 were counterbalanced (half of participants started with office). Training (2) was done in the respective starting block scenario (with or without office). \\
% Datasets were randomized between all 30 trials.\\



%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/Method21Konstanz/TaskCompletionTime.PNG}
%    \caption{Caption: results, Matthias; Participants required more time to complete the comparative visual exploration task when the environment was looking more realistically}
%    \label{fig:Konstanz-results}
% \end{figure}

\paragraph{\textbf{Results and Discussion:}}
%For each trial, we measured four dependent variables, including the distances from the pointer location to the two ground-truth common peaks ($D_1$, $D_2$), the task completion time ($T$), and the number of layer movements during the trials ($N_m$). The participants were allowed to take as much time as they wish to complete the task.
Fig. \ref{fig:Konstanz-Barcharts} shows the results for our dependent variables across 180 trials for \plain{} and \real.
%From Fig.~\ref{fig:Konstanz-Barcharts}(a,b), we see that most distance measures fall within $0$-$0.07m$ (see inset). We also notice that that accuracy values in \plain{} are closer to $0$ than in \real. 
We define \textit{task accuracy} as the fraction of user selections  that deviate by a maximum of 5cm from the correct position. Fig. \ref{fig:Konstanz-Barcharts}(left) shows that \textit{task performance} for \plain{} (95\%) is slightly higher than for \real{} (92\%). %, while a two-tailed $t$-test indicates no statistical significance when comparing . \ben{why t-test when comparing just two measures? You cannot compare distributions here?}. 
As shown in Fig.~ \ref{fig:Konstanz-Barcharts}(center), average \textit{task completion time} for \plain{} ($32.5$s) is lower than for in \real{} (40.6 sec). A two-tailed $t$-test indicates that this variation is statistically significant ($p < 0.01$).
Interestingly, the task completion time does not appear to correlate with the amount of layer movements made.
Fig.~\ref{fig:Konstanz-Barcharts}(right) shows the \textit{number of layer movements} for \plain{} and \real. We found slightly more movements in \plain{} while most trials do not feature any movements. About 17\% of the trials in \plain{} are with movement compared to only 9\% of trials in \real. The two-tailed $t$-test indicates that this variation is statistically significant ($p \approx 0.03$).

Because participants were allowed to take as much time as they wish to complete a task, we anticipated that accuracy would be similar. We were intrigued by the two opposite indications by the average \textit{task completion time} and the \textit{average layer movement}. We considered the following explanations:
 \textit{(i)} \real{} provided more visual distractions than \plain. We would have expected more layer movements in \real{} as participants had to overcome perceptual distractions with the background. However, we recorded a slightly higher number of layer movements in \plain{} (+0.8\%). It is possible, that in \real, participants compensated possible distractions in another way, e.g., by changing their viewing position onto the visualization. 
  \textit{(ii)} The distraction caused by the office background may have increased the difficulty of the task, leading participants to take more time to ascertain their judgment. For \textit{task completion time}, our results provided some supporting evidence for the initial guideline \textit{``Rule \#7: Don't Replicate the Real World''}. In terms of the layer movement and the increase of interaction effort, our results reject \hii. However, we can observe that the cost of interaction is not always directly translated to the cost of task completion time. 

%Study II does not provide significant evidence to support or contest the general guideline posed by Niklas Elmqvist. However, it provides a first basis to build on in future research, considering only one aspect of replication: the surrounding environment in VREs.
%Moreover, it's providing a range of data to contest a \textit{subset} of Elmqvist's thesis while focusing on visual background and surrounding environment. 
\paragraph{\textbf{Implications:}}
Our results may inform a discussion about the \textit{scope} of the initial guideline with respect to both, virtual environments and to which parts the `reality' aspect applies to.
It provides a first basis to build on in future research, considering only one aspect of replication: the surrounding environment in VR environments. For example, based on our results, we can create a new guideline: \textit{``Reduce distraction and visual clutter in the background of VR environments to support the visual perception of information in the visualization''}. Further research is needed to study this new guideline as well as other cases and factors mentioned in Elmqvist's initial guideline.
%Clearly, according to grounded theory, further data collection is required to study both guidelines discussed in this section. 
%\alex{was there any follow-up on this direction? paper?}. mk: not yet


==> sections/OldTexFiles/coding.tex <==
\section{Coding and Categorization}
\label{sec:VisGuides}
%\ben{ben, alex draft}
%\newcommand{\xx}{\textcolor{red}{XX}}
\newcommand\perc[1]{\the\numexpr#1*100/217\%}
\newcommand{\says}[1]{\textit{`#1'}}
\newcommand{\xx}{\textcolor{red}{59}}

In this section, we focus on research questions \textbf{Q1} asking about \textit{how guidelines are used in the forum}.  
Based on traditional methods from GT such as \emph{open coding}, \emph{axial coding}, and \emph{selective coding}--- repeated through four iterations---we derived a categorization scheme with six dimensions (Fig 2). Two researchers acted as the main coders with the help of six other researchers. All coding was done on the data set \dataset{} (347 posts), which included all posts from \swansea (148 posts), and \zurich (40 posts), as well as additional posts posted on the forum without specific instructions (59 posts). 
Coding was applied individually to each forum post. 
We defined the post as the smallest unit where a person could enclose and elaborate a thought on the forum. 
Threads contain one or more posts, posted at different times and in different contexts which usually lead to a more complex, diverse, and heterogeneous structure.
Details about the coding process are found in Appendix A.4.
%These categorization variables only consider a kind of hierachy of topics. So, we reworked the categorization to support our investigation into the aforementioned research questions, using GT. 

%We used the GT methodology to formulate a categorization scheme for the data sets $D_{20190313}$ and $D_{\text{Swansea2019}}$.
%We used the scheme to code an updated dataset $D_{20200222}$, containing $D_{20190313}$, $D_{\text{Swansea2019}}$, and $D_{\text{UZH2020}}$, with a total of \FIXME{288 posts}.
%\EDIT{We used this schema to code the new course dataset: $D_{\text{UZH2020}}$}

% --------------
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/coding-stats.pdf}
    \caption{Distribution of the categories of the 347 posts in \dataset{}.}
    \label{fig:catstats}
    \vspace{-4mm}
\end{figure}

% Our GT coding process resulted in a categorization scheme that is described in detail in Appendix A. For the self-containment, we briefly summarize the scheme here. 

\subsection{Classification Scheme}

Our classification scheme consists of six dimensions, each with between 3-5 categories, including one category for \texttt{unclear/none}:

\begin{description}[noitemsep]
  \item [D1:] \textbf{Main Purpose} describes the main purpose of a post. If a post exhibits more than one purpose, the coder made a judgment about what the main one is. The dimension's categories include \emph{Ask for Advice}, \emph{Offer Advice}, \emph{Discuss Guidelines}, \emph{Seek Clarification} (e.g., ``Please explain X'', \emph{Add Classification}, \emph{Social Conversation} (e.g., ``Thank you''), and \emph{Administration}.

  \item [D2:] \textbf{Guideline Mentioning} describes \textit{if} and \textit{how} a post mentions a visualization guideline. Its categories include \emph{Direct} (a guideline is explicitly mentioned in the post), \emph{Indirect} (a reference is given and it likely contains one or more guidelines related to the post), \emph{Implicit} (a reasonably well-known guideline can be identified by the coder), \emph{Unclear or Possible} (the coder is uncertain), and \emph{None} (the coder is certain that there is no guideline).

  \item [D3:] \textbf{Evidence} grades the level of detail of any supporting evidence given in a post. Its categories include \emph{Detailed}, \emph{Brief} (typically relying on references), \emph{Unclear}, and \emph{None}.

  \item [D4:] \textbf{Main Scope} describes the generality of the discourse in the post in terms of its applicability. Its categories include \emph{Case-based} (focusing on one or more individual cases), \emph{Conditional} (applicable to a number of cases under certain conditions), \emph{Contextual} (focusing on a high-level context, e.g., a topic, a type of tasks, a type of users, etc.), \emph{General} (applicable to most visualization contexts), \emph{Unclear}, and \emph{None}.

  \item [D5:] \textbf{Antithesis} describes the stance of a post with respect to all previous posts in the thread. Its categories include \emph{Neutral} (no opinion expressed), \emph{So Far So Good} (agreeing with all previous posts), \emph{Objection} (disagreeing with at least one previous posts), and \emph{Unclear}.

  \item [D6:] \textbf{Conviction} classifies the level of conviction shown by the arguments in a post. Its categories include \emph{Neutral} (no opinion expressed), \emph{Doubtful} (expressing some doubts), \emph{Suggestive} (suggesting an opinion with some uncertainty), \emph{Affirmative}, and \emph{Unclear}.
\end{description}

In addition to these six dimensions, we extracted most of the directly and indirectly mentioned guidelines from the 347 posts. These guidelines are listed in Appendix B.

%-------------
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/pcp.pdf}
    \caption{Visualizing the relationships among different variables. Red lines are associated with the category of \emph{Discuss Guidelines}, while the blue lines are associated with that of \emph{Offer Advice}.}
    \label{fig:catpcp}
    \vspace{-4mm}
\end{figure}


\subsection{Results and Findings}

Fig.~\ref{fig:catstats} summarizes the distribution of posts in \dataset, using our classification scheme. While the exact numbers naturally differ in subsets of the dataset, such as \zurich{} and \swansea{} and thus may be hard to generalize to other data sets and collection methods (see Section 4), our coding helps us to address \textbf{Q1}. Fig.~\ref{fig:catpcp} compares how guidelines are mentioned by posts that \emph{Offer Advice} (blue lines) and those that \emph{Discuss Guidelines} (red lines), revealing that most posts offering advice do not mention guidelines neither directly nor indirectly. 

From the coded data, the statistics, and the visualizations, we made the following observations.

\textbf{Using and discussing guidelines is not as common as one would prefer to see (D1).} Figure \ref{fig:catstats} shows that 32\% of the posts are in the D1 categorizes of \emph{Ask for Advice} and 35\% in \emph{Offer Advice}, while about 16\% are in the category of \emph{Discussing Guidelines}. We conjectured a few possible reasons: 
(i) recalling guidelines precisely may be difficult without a structured repository of guidelines; (ii) discussing guidelines may require broad or in-depth knowledge about visualization; (iii) applying some guidelines to practical problems may be easier said than done when one does not know the applicable conditions of a guideline.

\textbf{Few posts explicitly state guidelines (D2).}  Few posts proposed new guidelines or made abstraction or generalization from individual scenarios. About 58.5\% of the posts do not mention any guideline at all, much higher than the 26\% that mentioned guidelines directly and indirectly. Appendix B shows that a total of 14 guidelines were directly mentioned, and another 15 references were mentioned as support to some discussions.
%% AD: update guidelines

\textbf{Few posts provide reference to evidence (D3).}
Many posts provided example cases and detailed explanations about the reasons behind an advice (55\%). However, few posts mentioned references to the sources of guidelines such as scientific papers of textbooks (D2). %The most common reference was to ColorBrewer~\cite{brewer1994color}, which perhaps has a quasi-guideline status due to its wide acceptance and utilization. 
%Our finding indicates that it is easy to talk about details, taxing to mention references, and difficult to abstract and generalize. 

\textbf{It has been rare to discuss the conditions where a guideline may or may not be applicable (D4).} Typically (17.5\%), posts are contextual rather than conditional (5\%), while a large majority focuses on the specific case mentioned in the first post of a thread (60\%). 

\textbf{Few posts pose critical questions or offering critical comments (D5, D6).}
Fig.~\ref{fig:catstats} shows that about 89\% of the posts did not voice any objection against any opinions in the previous posts, while only 11\% featured disagreement (objection). About 30\% the posts were shown to be neutral in offering opinions, while those that did offer views typically used a suggestive tone (D6, 26\%). 

%% AD: I chopped the "prevalence of topics". I found it irrelevant because it is just a setup. We defined them, and then did an exercise about visual design. Therefore, it is not news that "visual design" is going to prevail.
%\textbf{Prevalence of topics} based on self-chosen keywords. Most posts are on the topic of \textit{Visual Design} (79.8\%). The rest of the posts are sparsely distributed among the other 10 topic categories, including \textit{Perception} (6.0\%), \textit{Education} (2.8\%), \textit{Theory} (2.4\%), \textit{Interaction} (2.0\%), \textit{Uncategorized} (2.0\%), \textit{Cognition} (1.6\%), \textit{General} (1.2\%), \textit{VR/VE} (0.8\%), \textit{Site Feedback} (0.8\%), and \textit{Medical Visualization} (0.2\%). VisGuides consequential offered subcategories for \textit{Visual Design}, each attracting 2.0\% or less. These number indicate that topic keywords in VisGuides need to be refined. To our best knowledge, there has not been a topic categorization scheme proposed for visualization topics in the literature. Further research to develop taxonomies or ontologies of visualization guidelines is urgently needed.

Our scheme and the results show that coding strategies are helpful in understanding how people address guidelines. However, the real challenge, learned from this data and from engaging students in using the forum (Section 4) is to systematize the \textit{use} and \textit{discussion} of guidelines. These efforts on education on guidelines, their uses and limitations (Section 4) were useful and helpful to bridge the gap towards a ``culture of guidelines'', their curation, discussion and critique.
This can start in our visualization classes, but needs broad buy-in from academics and practitioners, echoing some of the initiatives for collecting guidelines centrally~\cite{Scott-Brown2018Presenting}.


% \textbf{Detail is given, but references are missing.}
% Many advice in the forum contained sound insight and detailed explanations about the reasons behind an advice. We think this is very positive given that posting in the forum is voluntary. Most explanations contained examples and explained the reasons behind their advice while in other cases, a brief answer is everything it takes to solve a question. Few posts only contained pointers to scientific references and guidelines (). The most common reference we found was to ColorBrewer (), which can be seen as having quasi-guideline status in the visualization community due to its standardized and evidence-based color scale templates. However, we also found that very few people formulating their own guidelines when giving advice. Many posts do not make abstraction or generalization, especially when answering to posts that mention specific cases (seek-advice, give-advice). We believe formulating guidelines, even for very specific cases, can help building `thinking in guidelines' that go beyond specific advice for a specific case. 

% Most posts in the forum were asking for advice on very specific cases and replying to such cases (H1), while directly quoting guidelines is not common. Fewer posts (20.74\%) actually discussed guidelines. While this is largely due to the class assignment (Section XX), discussing guidelines is a complex job. If the goal of an advice is to advice in a specific case, it often is sufficient and pragmatic to link to a guideline, state it, or imply it. Though adapting a guideline to a specific case can sometimes be non-trivial and requires discussion, this does not necessarily require knowing all the evidence and expressing total faith in a guideline. Discussing a guideline, in public and with one's name attached, requires more effort and confidence. Discussing a guideline in depth, requires a broad understanding of the specific area of visualization (color theory, 3D visualization, perception, tasks), especially since most cases stretch across fields. It requires knowledge of the literature and the respective evidence as well as cases and examples in order to provide a critical in-depth discussion about the guideline's scope, limitation and how to correctly apply it. In fact, most of the in-depth discussions in the VisGuides forum come from experts in the field of visualization. 

 
% \textbf{A central repository could help building a culture around guidelines.}
% Other possible reasons for people refraining from using guidelines might include that there is no central repository on guidelines. Such a repository could help establish agreement and help to popularize guidelines as well as increase confidence in using certain guidelines is undermined by missing evaluations. Ideally, such a repository would come in a structured way and includes formulations, references, possible variations, but most importantly the discussions themselves. While part of our research question was to see if and how agreement about guidelines can be established, we require more data and discussion. Of course, such a repository, in part outlined by Scott-Brown~\cite{Scott-Brown2018Presenting}, would require a culture around guidelines that includes use, formulation, evidencing, scoping, and discussing. 

% \textbf{Something about discussions here.} Similar may hold for posing questions about guidelines. A large part of the questions we received in the forum ask for very advice on a specific to a varying degree. Some posts very openly asked for `advice' and if a visualization design could be improved. Others replied in more detail and only a tiny fraction () included a guideline in their question. A much smaller fraction () of questions explicitly asked for discussing a specific guideline. Being able to pose a critical question about a guideline requires a broader understanding and expertise. However, the number of posts asking for advice on guidelines in the case of a specific visualization shows that an easy way to start a discussion is to question the application and interpretation of a guideline in a specific example case. 

% \textbf{Towards more data and theories.} In summary, the findings from our open coding provide for some discussion and we found our categorization scheme rooted in Grounded Theory to answer our research questions. To generalize and extend our findings, more data is necessary. Through our iterations, we abandoned some dimensions as we found them to require more discussion and definition and data to be truly `grounded'.

% \textcolor{red}{=======OLD DRAFT BELOW======}

% \subsection{Categories}

% Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

% \textbf{A1: Type of Question}---This aspect describes the question and what the question is asking for. We found that most questions either asked for help for a specific visualization problems, wanted to discuss a specific guideline (`Don't replicate the real world'), or asked for guidelines around a specific topic (e.g, 3D visualization).

% \begin{itemize}[noitemsep]
%     \item \textbf{Guideline seeking:} A question looking for guidelines for a specific topic or problem. For a specific problem, the post-creator does not know a guideline or there are no guidelines. Examples include \xx.
%     \item \textbf{Guideline use:} a question looking how to employ a specific guideline or asking how to exactly interpret this guideline.
%     \item \textbf{Guideline critique}: a guideline is posted (or referenced) and put into question. This requires some argument, motivation, and reason for questioning the specific guideline.
%     \item \textbf{Guideline scope}: a question that asks if a particular guideline is valid in a given case and how to apply the guideline for this specific case.
%     \item \textbf{Design choices}: a question that posts a specific piece of visualization, asking the audience for advice on its design. Some questions ask about specific design choices (\says{Are the colors I have chosen alright}{2})
% \end{itemize}

% \textbf{A2: Type of Advice}---This aspect describes what type of advice was given, posted as answers to a question. We found a great variety in the types of replies and decided to settle on the following ones. A more fine-grained categorization might be possible but is out of scope of this paper as (a) this would require a very detailed investigation of the language used, and (b) would help less to answer our specific hypotheses as stated above.

% \begin{itemize}[noitemsep]
%     \item \textbf{Guideline}: a reply that states a guideline as answer to the question. For example \xx.
%     \item \textbf{Critique}: a reply that states and explains a critique to the guideline in question or uses guidelines to critique an initially posted visualization, example, or guideline. Examples include \xx.
%     \item \textbf{Clarification/Elaboration}: a reply that clarifies, elaborates, or defends a previously mentioned guideline. This can include delivering arguments in favor of the guideline or detailing its use and meaning. Examples include \xx.
%     \item \textbf{General Discussion:} some replies contained discussions that went beyond an individual guideline while discussing other and often more general topics. One example was \says{To make good design choices, we must understand visual perception: what works for the human brain, what doesn't, and why. We develop this ability through study and practice. Asking questions, as you have, is an essential part of this process.}{Few}. 
%     \item \textbf{Suggestion:} a reply that made suggestions to question or proposed solutions to a stated problem. Suggestions were very common and contained suggestions about visual encodings (\says{}{}), tools (\says{[...] use a series of sequential ``single hue'' colors maps [...] in ColorBrewer}{}) visualizations (\says{You should also consider using a glyph}{x})
%     \item \textbf{Instructive Question}
%     \item \textbf{Statement/Fact}
% \end{itemize}

% \textbf{A3: Specificity}---This aspect describes how specific an advice was given, independent from the type. 

% \begin{itemize}[noitemsep]
%     \item \textbf{Specific} advise on how to implement a guideline or how to solve a specific problem such as \says{}{}.
%     \item \textbf{General} advise on a guidelines or independent from an actual case such as such as \says{}{}. 
% \end{itemize}

% \textbf{A4: Evidence}---
% \begin{itemize}[noitemsep]
%     \item \textbf{Publication} includes any scientific publication or text book published through a process that assures some sort of rigor such as peer review, public opinion, or credible experience. Compared to the other categories for this aspect, \textit{Publications} are both traceable and highly credible. Ideally, each reply would use publications as reference, but lack of publications for making a specific point makes this hard. 
%     \item \textbf{Web source} includes blogs and websites of both credible sources (Niklas' blog, ColorBrewer) but also less strict and more popular sources such as \xx. 
%     \item \textbf{Discussion} includes any reference to a public discussion in a forum, another thread in VisGuides or on Twitter. 
%     \item \textbf{Experience/Opinion} include anything that comes from less referable sources such as a participants opinion or experience. Tracing evidence in these cases is possible, but credibility might be low.
% \end{itemize}


% \textbf{A5: Guidelines}---

% \textbf{A6: Topics}---For each thread, we coded \textit{specific} and \textit{general} visualization topics. 
% \begin{itemize}[noitemsep]
%     \item \textbf{Specific} topics included those explicitly mentioned in the text. Examples include \textit{use-of-color}, \textit{color-schemes}, \textit{human eye-brain system models}, etc. (For a full list, see \xx.)
%     \item \textbf{General} topics include those inferred by the coders and referring to more general topics in visualizations. Examples of general topics include \textit{color}, \textit{perception}, \textit{VR}, \textit{interaction}, \textit{learning}, \textit{visual effects}, \textit{3d-visualization}, \textit{2d-visualization}, \textit{cognitive load}, \textit{spatial-data}, \textit{design}, \textit{readability}, \textit{theory-models}, \textit{labeling} (1), and \textit{design} (2).
% \end{itemize}

% \textbf{A7: Agreement}
% \begin{itemize}
%     \item \textbf{Agreement} means that discussion participants agreed on an issue or guideline. 
%     \item \textbf{Partial agreement} 
%     \item \textbf{N/A}
% \end{itemize}


==> sections/OldTexFiles/discussions.tex <==
\label{sec:Conclusions}
%
In this paper, we have reported a set of GT-based methods (Table 1) for grounding our understanding of visualization guidelines on data collected from our online forum VisGuides. 

Through mainly \textit{coding} and \textit{categorization} we could develop a categorization scheme for analyzing guideline discussions (Section \ref{sec:VisGuides}) and could find guidelines, modes of discussion, the ways guidelines were mentioned and how specific arguments in the forum were backed up by examples, references, and empirical data. To complement this close reading, we used text analysis methods (Section \ref{sec:TextAnalytics}) to find structures in the data, such as clusters and potential hierarchies of concepts which might inform future guideline and topic taxonomies to support categorization, retrieval, and systematization of guidelines for storage, browsing, and teaching. Informed by guidelines and discussions posted online, our two controlled user studies (Section \ref{sec:EmpiricalStudies}) provide empirical evidence to contest, amend, and specialize existing guidelines and potentially generate new guidelines. Our methods are complementary in that they address different goals (categorization, groups, analysis) and methods for data collection (coding, automatic analysis, controlling factors, quantitative data). This methodology facilitates different insights about guidelines such as \textit{which} guidelines exist, how are guidelines \textit{discussed}, how are \textit{cases} cited, which \textit{factors} are included in a guideline, what \textit{empirical data} is available, and the role of empirical studies.

During our research, we appreciated not only the systematic approach advocated by GT for grounding the answers to research questions on data collection, categorization, and analysis, but the emphasis of GT for \textit{continuing investigation} until theoretical saturation. While reaching theoretical saturation is a long-term effort based on many studies and investigations that can only be carried forward by a collaborative scientific community, we believe our studies can provide examples for studying guidelines in visualization. 
In addition, when more data comes available, further examination of the use of guidelines in different contexts, and further empirical studies for evaluating guidelines should be performed for improving our categorization scheme.
We consider it desirable for the visualization community to make a collective effort to increase the mention and discussion of guidelines, especially in offering advice. 
One necessary step for enabling such effort is to maintain a unified repository for storing guidelines, creating suitable taxonomies or ontology for aiding the categorization and retrieval of guidelines, as well as structured methods~\cite{huron2020visactivities} to include guidelines in teaching (Section~\ref{sec:Teaching} alongside appropriate teaching material such as forums, repositories, browsing interfaces, and reports~\cite{abdul2020visguides}).

==> sections/OldTexFiles/intro.tex <==
A plethora of \textit{guidelines} for visualization have been recommended in books, research papers, and online media~\cite{kandogan2016grounded}. Examples include Tufte's Data-Ink ratio~\cite{tufte2001visual}, to `avoid the rainbow color map'~\cite{borland2007rainbow}, or to `carefully use visual embellishment'~\cite{bateman2010useful}. Most guidelines are based on authors' experience in designing and producing visualization imagery or on findings obtained from empirical studies. Guidelines aim to inform visualization design and application as well as to compress and render the ever-growing and fairly complex knowledge in visualization accessible, memorable, and applicable. In a sense, we can define a \emph{visualization guideline} to \textit{``embody wisdom advising a sound practice for designing and producing visualization imagery in practical applications.''} This can include best practices, taxonomies and ontologies, or models in visualization with keywords and causal relations~\cite{Chen:2017:CGA}. If a guideline is defined properly and with rigour, it is invaluable to both practical applications and the theoretical foundation of visualization.

%% talk about problems of using and formulating guidelines
Of course, it may not be trivial to define and describe every guideline precisely. To render guidelines applicable, there must be a tradeoff between describing a guideline together with detailed specifications of applicable and inapplicable conditions on the one side and making it general and memorable on the other side. Some guidelines may even be in conflict with one another. All of this is acceptable if there is evidence and agreed-on examples that support each guideline and justify its application. Thus, if visualization guidelines are to play a credible role in any mission-critical data analytics, knowledge discovery, design, or decision making workflow, then they must be rigorously evaluated, critiqued, and maintained, such as, for example, how guidelines in medical or healthcare would be scrutinized.

To help understanding how we can create better guidelines for visualization, this paper proposes a set of methods---i.e. a methodology---to study visualization guidelines using \textit{Grounded Theory}. Grounded theory (GT) is a well-established methodology in social science to scrutinize a postulated theory and was first proposed by Glaser and Strauss for sociological research \cite{Glaser:1967:book} 
by \textit{grounding} it in data. \alex{In this paper, we follow the methodological GT school of Strauss and Corbin, and the extensions in Constructivist GT. More details can be found in the Appendix D. }
GT requires a set of reliable recordings (data) that can be used to inform and ground any subsequent theory through methods such as \textit{categorization}, \textit{coding}, \textit{memoing}, \textit{examples}, and others (Table 1). Naturally, any grounding and scrutinizing process and any subsequent theory or deductions depend on the quality of the data. 
%In this paper, we explore two very different approaches to systematically collect data about guidelines in visualization. On one side, and as suggested by GT, we can data can be collected by ``listening to people'' and how they talk about guidelines. For such \textit{anecdotal} evidence, we designed an online forum \textit{VisGuides} (\url{http://visguides.org})~\cite{Diehl:2018:EuroVis} in which participants could freely discuss advice and guidelines in visualization. This approach is based on observations, categorizations, cases, references etc. On the other side, we can follow \textit{empirical} approaches, commonly used in Human-Computer Interaction and visualization research, to prove of disprove specific guidelines and theories, formulated in the anecdotal approach. Empirical studies set out to study guidelines in a controlled setup an with clear hypotheses in mind. While we employed traditional GT processes, we also utilized our own expertise in computer-assisted data analysis and visualization to complement the traditional processes (Table 1).

\alex{To provide for a reliable source of data, the methods in this paper are organized around an online forum \textit{VisGuides}~\cite{Diehl:2018:EuroVis} (\url{http://visguides.org}) meant for discussing visualization guidelines and which provides us with data about the use and discussion of visualization guidelines in different contexts. 
We acknowledge the existence of other popular forums such as the subreddit `Data is beautiful'~\cite{data-is-beautiful:2020} and the discussions on the Data Visualization Society slack channel~\cite{DVS:2020}, as well as many other blogs and personal web-pages. 
Nevertheless, they are not needed for the especification of our methodological framework. 
Our approach includes the iteration over new data sets, such as the ones mentioned before, as an iteration of the GT methodology using new data sets, aiming at the theoretical saturation of theories of guidelines (see Fig.~\ref{fig:teaser}). }
For this paper, we use data from 33 continuous months between September 1st, 2017 and February, 22nd, 2020. To analyze this data we present different methods and processes stipulated by GT and address the following research questions:

\begin{description}

\item [Q1:] \textit{If and how are visualization guidelines mentioned and discussed in VisGuides posts?}
%\ben{To methodolgy: We manually coded and categorized posts to describe purposes of posts, which evidence was given to support an advice and what the scope of each post was. This lead us to categories for...} (Section 4)
\item [Q2:] \textit{What can automatic concept extraction tell us about \alex{the formulation and discussion} of visualization guidelines?}
\item [Q3:] \textit{
%Which guidelines lack empirical knowledge and 
How can controlled user studies contribute to defining and contesting guidelines?} 
\item [Q4:] \textit{How \alex{are guidelines formulated and discussed in the students' conversations and how the discussion of guidelines affect the understanding of visualization in teaching contexts?}} 
%and which visualization guidelines mentioned in the forum could be included in the lectures on data visualization?} While engaging with the 
%\EDiT{We analyzed the results of the discussion of guidelines in the VisGuides forum, in the context of education. We performed two studies in the educational context. First, a pilot study in 2019 in a British University visualization course, and then, a follow-up study in 2020 in a Swiss University visualization course, where we incorporated the lessons learned from the first pilot.   (Section~\ref{GT_education}).
\end{description}

By rigorously applying techniques from GT (Section~\ref{sec:VisGuides}) and complementing traditional methods with computer-aided methods (Section~\ref{sec:TextAnalytics}) and controlled user studies (Section~\ref{sec:EmpiricalStudies}), we provide the following contributions: 
\begin{itemize} %[noitemsep]
    \item  A set of multifaceted methods to study visualization guidelines according to GT, %as part of the theoretical foundation of visualization \cite{Chen:2017:CGA}
    \item A methodology to enrich traditional methods in GT through digital technologies such as web forums, data visualization, text analysis, and controlled empirical studies.
    \item As part of our methodology, we exemplify and provided further evidence to support two visualization guidelines, uncovered a number of guidelines buried in the literature, and identified several challenges and opportunities for attaining theoretical saturation.
\end{itemize}

Findings from our research \alex{build a theoretical and methodological scaffolding for the theoretical formulation, understanding, and scrutinizing of visualization guidelines},
%help building a better understanding of how to collect data about guidelines, how to scrutinize guidelines, 
and extend our community's  repertoire of research methods for guidelines beyond the traditional framework proposed by GT.




==> sections/OldTexFiles/opencoding-old.v1.tex <==
\section{Categorization and Coding}
\label{sec:VisGuides}
%\ben{ben, alex draft}
%\newcommand{\xx}{\textcolor{red}{XX}}
%\newcommand{\says}[2]{\textit{``#1''}{(#2)}

VisGuides was launched on September 27, 2017 \cite{Diehl:2018:EuroVis}. There were 238 posts up to March 13, 2019 when we collected the latest data set $D_{20190313}$ for the analysis in this paper. The data set contains discourses on some prevalent topics (e.g., color, interaction, virtual reality (VR), and so on), and contributions from users with many different visualization backgrounds, ranging from undergraduate students to highly-respected visualization experts (e.g., in alphabetic order, Niklas Elmqvist, Stephen Few, Eduard Gr\"{o}ller, Theresa-Marie Rhyne, Bernice Rogowitz, and so on).
One cannot help wonder if this data set would inform some ``theories''.Following the tradition in the field of visualization, we use the terms such as ``research questions'', ``hypotheses'', ``categorization schemes'', and ``findings'' instead of ``theories'' in the following discussions.

In this section, we focus on several holistic research questions about visualization guidelines, including
(i) whether and in which way were guidelines mentioned in the posts,
(ii) which guidelines were mentioned and how did the relevant posts discuss them, and
(iii) how should guidelines be categorized?
As $D_{20190313}$ consists of primarily free texts, any answers about ``whether'', ``in which way'', ``which'', and ``how'' depend critically on the interpretation of the texts. From the perspective of grounded theory, the key to befitting interpretations is a correct categorization and coding.

% This section reports on our open coding from XX forum threads. A thread is a question and its answers. Goal of the our open coding was to better understand the use of guidelines in the forum.

Because VisGuides is a computer-assisted platform, the computer has to some extend provided some categorization schemes and automated coding (or selective coding in a grounded theory term). These include those variables in Table \ref{tab:A1-A8} for coding each post. Clearly, these categorization variables would not be sufficient for supporting our investigation into the aforementioned research questions. 

\paragraph{\textbf{Grounded Theory Process.}} \textcolor{red}{TODO}

\paragraph{\textbf{Variables and Categories.}} \textcolor{red}{TODO}

\paragraph{\textbf{Findings.}} \textcolor{red}{TODO}

\textcolor{red}{CURRENT DRAFT BELOW}

\subsection{Methodology}

Our methodology followed several iterative open coding cycles. First, two of the paper authors started reading a random set of around 5-9 articles and tagging them according to information that could potentially be relevant to our questions. Then, the same two authors discussed possible aspects for tagging such as ``what are questions asking for'', ``how specific are they asking for advice'' or ``which guidelines are mentioned in the threads''. For each aspect, we started to formulate categories that we could use to tag a thread. We then asked a third coder to join and explained our aspects and categories to her. Then, each of the three coders individually coded the same set of 10 threads that received most answers (top-10). After coding, the three coders refined categories in each aspects to accommodate for disagreement and diverging interpretations. Finally, one coder went ahead coding another set of \xx threads.

\subsection{Categories}

Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

\textbf{A1: Type of Question}---This aspect describes the question and what the question is asking for. We found that most questions either asked for help for a specific visualization problems, wanted to discuss a specific guideline (`Don't replicate the real world'), or asked for guidelines around a specific topic (e.g, 3D visualization).

\begin{itemize}[noitemsep]
    \item \textbf{Guideline seeking:} A question looking for guidelines for a specific topic or problem. For a specific problem, the post-creator does not know a guideline or there are no guidelines. Examples include \xx.
    \item \textbf{Guideline use:} a question looking how to employ a specific guideline or asking how to exactly interpret this guideline.
    \item \textbf{Guideline critique}: a guideline is posted (or referenced) and put into question. This requires some argument, motivation, and reason for questioning the specific guideline.
    \item \textbf{Guideline scope}: a question that asks if a particular guideline is valid in a given case and how to apply the guideline for this specific case.
    \item \textbf{Design choices}: a question that posts a specific piece of visualization, asking the audience for advice on its design. Some questions ask about specific design choices (\says{Are the colors I have chosen alright}{2})
\end{itemize}

\textbf{A2: Type of Advice}---This aspect describes what type of advice was given, posted as answers to a question. We found a great variety in the types of replies and decided to settle on the following ones. A more fine-grained categorization might be possible but is out of scope of this paper as (a) this would require a very detailed investigation of the language used, and (b) would help less to answer our specific hypotheses as stated above.

\begin{itemize}[noitemsep]
    \item \textbf{Guideline}: a reply that states a guideline as answer to the question. For example \xx.
    \item \textbf{Critique}: a reply that states and explains a critique to the guideline in question or uses guidelines to critique an initially posted visualization, example, or guideline. Examples include \xx.
    \item \textbf{Clarification/Elaboration}: a reply that clarifies, elaborates, or defends a previously mentioned guideline. This can include delivering arguments in favor of the guideline or detailing its use and meaning. Examples include \xx.
    \item \textbf{General Discussion:} some replies contained discussions that went beyond an individual guideline while discussing other and often more general topics. One example was \says{To make good design choices, we must understand visual perception: what works for the human brain, what doesn't, and why. We develop this ability through study and practice. Asking questions, as you have, is an essential part of this process.}{Few}. 
    \item \textbf{Suggestion:} a reply that made suggestions to question or proposed solutions to a stated problem. Suggestions were very common and contained suggestions about visual encodings (\says{}{}), tools (\says{[...] use a series of sequential ``single hue'' colors maps [...] in ColorBrewer}{}) visualizations (\says{You should also consider using a glyph}{x})
    \item \textbf{Instructive Question}
    \item \textbf{Statement/Fact}
\end{itemize}

\textbf{A3: Specificity}---This aspect describes how specific an advice was given, independent from the type. 

\begin{itemize}[noitemsep]
    \item \textbf{Specific} advise on how to implement a guideline or how to solve a specific problem such as \says{}{}.
    \item \textbf{General} advise on a guidelines or independent from an actual case such as such as \says{}{}. 
\end{itemize}

\textbf{A4: Evidence}---
\begin{itemize}[noitemsep]
    \item \textbf{Publication} includes any scientific publication or text book published through a process that assures some sort of rigor such as peer review, public opinion, or credible experience. Compared to the other categories for this aspect, \textit{Publications} are both traceable and highly credible. Ideally, each reply would use publications as reference, but lack of publications for making a specific point makes this hard. 
    \item \textbf{Web source} includes blogs and websites of both credible sources (Niklas' blog, ColorBrewer) but also less strict and more popular sources such as \xx. 
    \item \textbf{Discussion} includes any reference to a public discussion in a forum, another thread in VisGuides or on Twitter. 
    \item \textbf{Experience/Opinion} include anything that comes from less referable sources such as a participants opinion or experience. Tracing evidence in these cases is possible, but credibility might be low.
\end{itemize}


\textbf{A5: Guidelines}---

\textbf{A6: Topics}---For each thread, we coded \textit{specific} and \textit{general} visualization topics. 
\begin{itemize}[noitemsep]
    \item \textbf{Specific} topics included those explicitly mentioned in the text. Examples include \textit{use-of-color}, \textit{color-schemes}, \textit{human eye-brain system models}, etc. (For a full list, see \xx.)
    \item \textbf{General} topics include those inferred by the coders and referring to more general topics in visualizations. Examples of general topics include \textit{color}, \textit{perception}, \textit{VR}, \textit{interaction}, \textit{learning}, \textit{visual effects}, \textit{3d-visualization}, \textit{2d-visualization}, \textit{cognitive load}, \textit{spatial-data}, \textit{design}, \textit{readability}, \textit{theory-models}, \textit{labeling} (1), and \textit{design} (2).
\end{itemize}

\textbf{A7: Agreement}
\begin{itemize}
    \item \textbf{Agreement} means that discussion participants agreed on an issue or guideline. 
    \item \textbf{Partial agreement} 
    \item \textbf{N/A}
\end{itemize}





\subsection{Findings}

In terms of grounded theory, this example points out some problems and a solution in visualization:

\begin{itemize}
    \item Common-sense advices seem to be a commonplace, and directly quoting guidelines are not common --- possible reasons: no central repository, no adequate evaluation, so lack of confidence for using them.
    \item Although many advices contain sound insight, and many do not make abstraction or generalization --- possible reasons: lack of confidence for defining them or lack of means for proposing them, discussing them, and evaluating them (i.e., not using the grounded theory methodology)
\end{itemize}




==> sections/OldTexFiles/opencoding-old.v2.tex <==
\section{Categorization and Coding}
\label{sec:VisGuides}
\ben{ben, alex draft}

%\newcommand{\xx}{\textcolor{red}{XX}}
% \newcommand{\says}[2]{\textit{``#1''}{(#2)}}

This section reports on our open coding from XX forum threads. A thread is a question and its answers. Goal of the our open coding was to better understand the use of guidelines in the forum.

(i) if and in which way guidelines are mentioned in the posts?
(ii) which guidelines are mentioned and how a post argues about them, and?
(iii) if and how guidelines are discussed and disputed in the posts?

\subsection{Research questions}


\subsection{Methodology}

Our methodology followed several iterative open coding cycles. First, two of the paper authors started reading a random set of around 5-9 articles and tagging them according to information that could potentially be relevant to our questions. Then, the same two authors discussed possible aspects for tagging such as ``what are questions asking for'', ``how specific are they asking for advice'' or ``which guidelines are mentioned in the threads''. For each aspect, we started to formulate categories that we could use to tag a thread. We then asked a third coder to join and explained our aspects and categories to her. Then, each of the three coders individually coded the same set of 10 threads that received most answers (top-10). After coding, the three coders refined categories in each aspects to accommodate for disagreement and diverging interpretations. Finally, one coder went ahead coding another set of \xx threads.

\subsection{Categories}

Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

\textbf{D1: Guideline mentioning:} \textit{Are there any guidelines mentioned in the reply and if so, how explicit is this guideline mentioned?} 

\begin{itemize}[noitemsep]
\item \textbf{Explicit:} A guideline is explicitly formulated with a clear advice what to do. Examples of explicit mentionings include \says{Avoid using visual effects in graphs}{15} and \says{Everything in a graph – all of its objects and their visual attributes – should support the graph’s purpose}{16}). Explicit mentioning can include guidelines that are commonly known (e.g, Sheiderman's mantra), or being formulated so that clear advice follows.
\item \textbf{Indirect:} a guideline is indirectly mentioned by pointing to a reference that contains the guideline. Examples include \says{Chapter 2 of [2] provides you with an application of color for labeling of nominal data and its perceptual properties.}{}. The guideline(s) itself are not mentioned explicitly in the reply and it is up to the reader to find and potentially chose. 
%\item \textbf{Implicit:} a guideline is not stated explicitly (nor is it referenced) but an expert in visualization could carefully infer a guideline. For example \says{Pie charts are difficult for the human eye to correctly perceive.} could be re-formulated into ``Avoid pie charts because they are hard to perceive correctly''. 
\item \textbf{No guideline:} the reply is not mentioning any identifiable guideline. This category includes a long list of posts giving very detailed advice, asking questions and making suggestions. These types of messages are captured by our dimension X.		
\item \textbf{Unclear:} the coder is not certain about whether this reply contains a guideline or not.
\end{itemize}


\textbf{D2. Suggestiveness:} \textit{How strong should the reader adhere to the advise?}. This dimension looks at the specific formulations in the post.

\begin{itemize}[noitemsep]
\item \textbf{Imperative:} advice is formulated to imply strict following. Examples include formulations such as 'must', 'do', 'do not', 'should' such as \says{[...] you should consider whether you really need to simultaneously depict them all in a single static image.}
\item \textbf{Indicative:}  (advice can be followed: may, likely, the easiest way?, could, it would, I would)
\item \textbf{Neutral:} (statements which do not allow to infer any suggestion about what to do and what not to do)
\item \textbf{Not-suggestive/informative:}
\item \textbf{Unclear:}
\end{itemize}




\textbf{3. Conditionality:} How conditional is the advice formulated

\begin{itemize}[noitemsep]
\item \textbf{Conditional-explicit:} advice/guideline is stated with a condition when it is valid/not valid and does so explicitly. The condition is stated explicitly.
\item \textbf{Conditional-implicit:} advice does not tell condition explicitly. The reader cannot tell if the guideline applies to them or not. 
\item \textbf{No condition mentioned:} advice/guideline is stated in a way that does not allow to infer when it is valid or not and if there are cases where a guideline is not valid. If there are conditions, the reader does not know.
\item \textbf{Contextual:} advice/guideline does not allow to be generalized easily from the way it is stated. That means that the only condition that make it true are the specific case
\item \textbf{unclear}
\item \textbf{not-applicable}
\end{itemize}




\textbf{4. Support / Backing:} how to we know that a stated advise/guideline is true?  

\begin{itemize}[noitemsep]
\item \textbf{Example:} example case is given to illustrate guideline
\item \textbf{Discussion:} discusses valid and invalid cases for guideline, aiming to provide pro and contra arguments
\item \textbf{Explanation:} explain why guideline should be valid.
\item \textbf{Scientific Reference:} includes an external reference (we have another dimension to classify those)
\item \textbf{Web reference:}
\item \textbf{Opinion:} states an opinion which does not imply if the advices is proven and how valid it is.
\item \textbf{None:} no justification given, just statementx
\item \textbf{Unclear}
\end{itemize}




\textbf{5. Generalizability:} How general is this guideline with respect to other issues in visualization? 

\begin{itemize}[noitemsep]
\item \textbf{General:} applicable to almost every case in visualization, e.g., visualization design, task scope, and conveys methodological meta knowledge about how to do things in visualization, design, reserarch in general. Advise is not specific to an area within visualization.
\item \textbf{Topic-specific:} applicable to specific cases of data, visualization, tasks, contexts, etc.
\item \textbf{Case-specific:} applicable to only this specific case, 'in your case' but not necessarily to other cases with the same problem.
\item \textbf{unclear}
\end{itemize}

\subsection{Findings}

In terms of grounded theory, this example points out some problems and a solution in visualization:

\begin{itemize}
    \item Common-sense advices seem to be a commonplace, and directly quoting guidelines are not common --- possible reasons: no central repository, no adequate evaluation, so lack of confidence for using them.
    \item Although many advices contain sound insight, and many do not make abstraction or generalization --- possible reasons: lack of confidence for defining them or lack of means for proposing them, discussing them, and evaluating them (i.e., not using the grounded theory methodology)
\end{itemize}




==> sections/OldTexFiles/opencoding-old.v3.tex <==
\section{Categorization and Coding}
\label{sec:VisGuides}
%\ben{ben, alex draft}
%\newcommand{\xx}{\textcolor{red}{XX}}
\newcommand\perc[1]{\the\numexpr#1*100/217\%}
\newcommand{\says}[1]{\textit{`#1'}}



% This section reports on our open coding from XX forum threads. A thread is a question and its answers. Goal of the our open coding was to better understand the use of guidelines in the forum.

In this section, we focus on several holistic research questions about visualization guidelines, including \textbf{Q1-Q3} stated in Section \ref{sec:Introduction}.

Because VisGuides is a computer-assisted platform, the computer has to some extend provided some categorization schemes and automated coding (or selective coding in a grounded theory term). These include those variables in Table \ref{tab:Computer} in Appendix A for coding each post. Clearly, these categorization variables would not be sufficient for supporting our investigation into the aforementioned research questions. 

\newcommand{\xx}{\textcolor{red}{XX}}

\paragraph{\textbf{The GT Coding Process.}}
%
We used the GT methodology to formulate a categorization scheme for the data set $D_{20190313}$, and used the scheme to code all 248 posts in the data set. Two researchers acted as the main coders with the help of from five other researchers. It took three iterations of \emph{open coding}, \emph{axial coding}, and \emph{selective coding} for us to derive the main categorization scheme with six variables (version 3), which was revised slightly to yield version 4.
The details of our GT coding process can be found in Appendix A.4.

% --------------
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/visguides-charts.pdf}
    \caption{Distribution of the categories of the 248 posts in $D_{20190313}$.}
    \label{fig:catstats}
\end{figure}

\paragraph{\textbf{Variables and Categories.}}
Our GT coding process resulted in a categorization scheme with six variables, which include:
%




Dimensions and categories were applied to reflect the main purpose behind a post. Our final dimensions and categories are as follows, with percentages shown in Fig. \ref{fig:catstats} and relations across categories in Fig. \ref{fig:catpcp} 

\begin{itemize}[noitemsep, leftmargin=*]
    \item \textbf{D1: Main Purpose} captures the main purpose of a post. If the post exhibits more than one purpose, the coder made a judgment about what is the main one. Our categories included
    \textit{Ask-for-advice}~(34\%) in which case a post stated a specific problem or visualization example and asked for advice on that problem or visualization; 
    38\% were classified to \textit{Offer advice} and which replied with some sort of advice; \textit{Discuss guidelines}~(\perc{43}) were posts that discussed a specific guideline, questioning their use or correctness.
    \textit{Seek clarification}~(\perc{9}) referred to posts asking for any clarification with respect to a previous post. Eventually, we categorized posts into \textit{social conversation}~\perc{6}, e.g., those thanking for an advice. 
    
    \item \textbf{D2: Guideline mentioning} describes if and how explicit or implicit a post mentions a guidelines. About 19\% of all posts \textit{direct}ly spelled out a well known guideline such as \textit{`Don't Replicate the Real World'}. \textit{Indirect} (12\%) mentions did not spell out the guideline but instead provided a reference, for example \says{Your visualization satisfies many of Stephen Few’s principles [1]'}. Other posts mentioned guidelines \textit{implicit}ly~(4\%) so that a coder could guess the guideline though it was not spelled out explicitly. Examples include \says{A legend is a great tool to aid any visualisation.} and \says{Pie charts are difficult for the human eye to correctly perceive.}. Almost the majority of posts~(51\%), however, did not mention any guidelines and about 14\% could not be classified with enough certainty by the coders.
    
    \item \textbf{D3: Evidence} describes the level of detail and evidence within a statement. Most of the replies (58\%) contained \textit{detailed} evidence by e.g., mentioning details and laying our opinions. Other statements were found to contain \textit{brief} explanations (35\%) with references that would require the reader to search for the detailed arguments and advice themselves. Only about 6\% of all posts did not contain any evidence at all. 2\% of posts could not be classified (\textit{unclear}). 
    
    \item \textbf{D4: Main Scope} describes the scope of the post with respect to how specific or generic is it. For example, the majority of posts was \textit{case-specific}~(64\%) talking about very specific cases and making it hard to generalize to other problems in visualization. 4\% of posts were classified as \textit{conditional}, giving more general advice but at the same time mentioning a specific scope: \says{I understand that the 3D effect for the bar chart [...] is not helpful. But when a chart has overlapping objects, I wonder if I can use some mild 3D effects [...]}. The other large part (25\%) in our data set were \textit{contextual} posts, i.e., posts talking about more general topics in visualization such as color scales, visual perception, interaction etc. 5\% posts were simpler `thank you' messages and could not be classified under any specific scope. 
    
    \item \textbf{D5: Antithesis} describes the stance of a post with respect to its prior post. For example, while only 8\% of the posts were found to have a \textit{neutral} stance, the vast majority 77\% was found to largely agree with the previous post (\textit{so-far-so-good}). While this category included all the initial posts in a thread, after removing them about XX\% of replies fell in this category. A smaller fraction of posts (14\%) contained major \textit{objections} with respect to a previous post. 1\% of posts could not be classified (\textit{unclear}).
    
    \item \textbf{D6: Conviction} classified posts according to how much an author was insisting on his answer to be carried out. 42\% of all posts were rather \textit{neutral}, while 11\% were found \textit{doubtful}, i.e., including some doubts about a guideline or opinion in a previous post. The largest share of posts were formulated in a \textit{suggestive} way (36\%), suggesting a specific action while about 10\% had an \textit{affirmative} character. One post was categorized \textit{unclear} as it contained a very brief call for clarification.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/pcp.pdf}
    \caption{PCP}
    \label{fig:catpcp}
\end{figure}

\subsection{\textbf{Findings.}} %\textcolor{red}{ben: WIP}

\textbf{Using and discussing guidelines is non-trivial.}
Most posts in the forum were asking for advice on very specific cases and replying to such cases (H1), while directly quoting guidelines is not common. Fewer posts (20.74\%) actually discussed guidelines. While this is largely due to the class assignment (Section XX), discussing guidelines is a complex job. If the goal of an advice is to advice in a specific case, it often is sufficient and pragmatic to link to a guideline, state it, or imply it. Though adapting a guideline to a specific case can sometimes be non-trivial and requires discussion, this does not necessarily require knowing all the evidence and expressing total faith in a guideline. Discussing a guideline, in public and with one's name attached, requires more effort and confidence. Discussing a guideline in depth, requires a broad understanding of the specific area of visualization (color theory, 3D visualization, perception, tasks), especially since most cases stretch across fields. It requires knowledge of the literature and the respective evidence as well as cases and examples in order to provide a critical in-depth discussion about the guideline's scope, limitation and how to correctly apply it. In fact, most of the in-depth discussions in the VisGuides forum come from experts in the field of visualization. 

\textbf{Detail is given, but references are missing.}
Many advice in the forum contained sound insight and detailed explanations about the reasons behind an advice. We think this is very positive given that posting in the forum is voluntary. Most explanations contained examples and explained the reasons behind their advice while in other cases, a brief answer is everything it takes to solve a question. Few posts only contained pointers to scientific references and guidelines (). The most common reference we found was to ColorBrewer (), which can be seen as having quasi-guideline status in the visualization community due to its standardized and evidence-based color scale templates. However, we also found that very few people formulating their own guidelines when giving advice. Many posts do not make abstraction or generalization, especially when answering to posts that mention specific cases (seek-advice, give-advice). We believe formulating guidelines, even for very specific cases, can help building `thinking in guidelines' that go beyond specific advice for a specific case.  

\textbf{A central repository could help building a culture around guidelines.}
Other possible reasons for people refraining from using guidelines might include that there is no central repository on guidelines. Such a repository could help establish agreement and help to popularize guidelines as well as increase confidence in using certain guidelines is undermined by missing evaluations. Ideally, such a repository would come in a structured way and includes formulations, references, possible variations, but most importantly the discussions themselves. While part of our research question was to see if and how agreement about guidelines can be established, we require more data and discussion. Of course, such a repository, in part outlined by Scott-Brown~\cite{Scott-Brown2018Presenting}, would require a culture around guidelines that includes use, formulation, evidencing, scoping, and discussing. 

\textbf{Something about discussions here.} Similar may hold for posing questions about guidelines. A large part of the questions we received in the forum ask for very advice on a specific to a varying degree. Some posts very openly asked for `advice' and if a visualization design could be improved. Others replied in more detail and only a tiny fraction () included a guideline in their question. A much smaller fraction () of questions explicitly asked for discussing a specific guideline. Being able to pose a critical question about a guideline requires a broader understanding and expertise. However, the number of posts asking for advice on guidelines in the case of a specific visualization shows that an easy way to start a discussion is to question the application and interpretation of a guideline in a specific example case. 

\textbf{Towards more data and theories.} In summary, the findings from our open coding provide for some discussion and we found our categorization scheme rooted in Grounded Theory to answer our research questions. To generalize and extend our findings, more data is necessary. Through our iterations, we abandoned some dimensions as we found them to require more discussion and definition and data to be truly `grounded'.







% \textcolor{red}{=======OLD DRAFT BELOW======}

% \subsection{Categories}

% Our final coding was divided into six \textit{aspects} (A1-A6), with 2-8 \textit{categories} each. Each thread in the forum was classified for all  aspects. If one of the replies could be classified in a certain category, the thread was classified. Thus, multiple categories per thread were possible and in section x, we report on the statistics \textit{per thread}.

% \textbf{A1: Type of Question}---This aspect describes the question and what the question is asking for. We found that most questions either asked for help for a specific visualization problems, wanted to discuss a specific guideline (`Don't replicate the real world'), or asked for guidelines around a specific topic (e.g, 3D visualization).

% \begin{itemize}[noitemsep]
%     \item \textbf{Guideline seeking:} A question looking for guidelines for a specific topic or problem. For a specific problem, the post-creator does not know a guideline or there are no guidelines. Examples include \xx.
%     \item \textbf{Guideline use:} a question looking how to employ a specific guideline or asking how to exactly interpret this guideline.
%     \item \textbf{Guideline critique}: a guideline is posted (or referenced) and put into question. This requires some argument, motivation, and reason for questioning the specific guideline.
%     \item \textbf{Guideline scope}: a question that asks if a particular guideline is valid in a given case and how to apply the guideline for this specific case.
%     \item \textbf{Design choices}: a question that posts a specific piece of visualization, asking the audience for advice on its design. Some questions ask about specific design choices (\says{Are the colors I have chosen alright}{2})
% \end{itemize}

% \textbf{A2: Type of Advice}---This aspect describes what type of advice was given, posted as answers to a question. We found a great variety in the types of replies and decided to settle on the following ones. A more fine-grained categorization might be possible but is out of scope of this paper as (a) this would require a very detailed investigation of the language used, and (b) would help less to answer our specific hypotheses as stated above.

% \begin{itemize}[noitemsep]
%     \item \textbf{Guideline}: a reply that states a guideline as answer to the question. For example \xx.
%     \item \textbf{Critique}: a reply that states and explains a critique to the guideline in question or uses guidelines to critique an initially posted visualization, example, or guideline. Examples include \xx.
%     \item \textbf{Clarification/Elaboration}: a reply that clarifies, elaborates, or defends a previously mentioned guideline. This can include delivering arguments in favor of the guideline or detailing its use and meaning. Examples include \xx.
%     \item \textbf{General Discussion:} some replies contained discussions that went beyond an individual guideline while discussing other and often more general topics. One example was \says{To make good design choices, we must understand visual perception: what works for the human brain, what doesn't, and why. We develop this ability through study and practice. Asking questions, as you have, is an essential part of this process.}{Few}. 
%     \item \textbf{Suggestion:} a reply that made suggestions to question or proposed solutions to a stated problem. Suggestions were very common and contained suggestions about visual encodings (\says{}{}), tools (\says{[...] use a series of sequential ``single hue'' colors maps [...] in ColorBrewer}{}) visualizations (\says{You should also consider using a glyph}{x})
%     \item \textbf{Instructive Question}
%     \item \textbf{Statement/Fact}
% \end{itemize}

% \textbf{A3: Specificity}---This aspect describes how specific an advice was given, independent from the type. 

% \begin{itemize}[noitemsep]
%     \item \textbf{Specific} advise on how to implement a guideline or how to solve a specific problem such as \says{}{}.
%     \item \textbf{General} advise on a guidelines or independent from an actual case such as such as \says{}{}. 
% \end{itemize}

% \textbf{A4: Evidence}---
% \begin{itemize}[noitemsep]
%     \item \textbf{Publication} includes any scientific publication or text book published through a process that assures some sort of rigor such as peer review, public opinion, or credible experience. Compared to the other categories for this aspect, \textit{Publications} are both traceable and highly credible. Ideally, each reply would use publications as reference, but lack of publications for making a specific point makes this hard. 
%     \item \textbf{Web source} includes blogs and websites of both credible sources (Niklas' blog, ColorBrewer) but also less strict and more popular sources such as \xx. 
%     \item \textbf{Discussion} includes any reference to a public discussion in a forum, another thread in VisGuides or on Twitter. 
%     \item \textbf{Experience/Opinion} include anything that comes from less referable sources such as a participants opinion or experience. Tracing evidence in these cases is possible, but credibility might be low.
% \end{itemize}


% \textbf{A5: Guidelines}---

% \textbf{A6: Topics}---For each thread, we coded \textit{specific} and \textit{general} visualization topics. 
% \begin{itemize}[noitemsep]
%     \item \textbf{Specific} topics included those explicitly mentioned in the text. Examples include \textit{use-of-color}, \textit{color-schemes}, \textit{human eye-brain system models}, etc. (For a full list, see \xx.)
%     \item \textbf{General} topics include those inferred by the coders and referring to more general topics in visualizations. Examples of general topics include \textit{color}, \textit{perception}, \textit{VR}, \textit{interaction}, \textit{learning}, \textit{visual effects}, \textit{3d-visualization}, \textit{2d-visualization}, \textit{cognitive load}, \textit{spatial-data}, \textit{design}, \textit{readability}, \textit{theory-models}, \textit{labeling} (1), and \textit{design} (2).
% \end{itemize}

% \textbf{A7: Agreement}
% \begin{itemize}
%     \item \textbf{Agreement} means that discussion participants agreed on an issue or guideline. 
%     \item \textbf{Partial agreement} 
%     \item \textbf{N/A}
% \end{itemize}







==> sections/OldTexFiles/overview.tex <==
\begin{table*}[t!]
  \centering
  \caption{A summary of the principles and methods of grounded theory, and an outlook on how computer-assisted implementation may complement the traditional implementation of the grounded theory (GT) methodology \cite{Willig:2013:book}.
  The section tags $\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:TextAnalytics}}$, $\S_{\ref{sec:Teaching}}$, and  $\S_{\ref{sec:EmpiricalStudies}}$ indicate those processes that were used in this work and detailed in the corresponding sections. The processes in \emph{italic} indicate possible future work. See also Appendix D.}
  \label{tab:GroundedTheory}
  
  \begin{tabular}{@{}p{3.2cm}@{\hspace{4mm}}p{7cm}@{\hspace{4mm}}p{7.2cm}@{}}
  \textbf{Methods and Principles} & \textbf{Traditional Implementation} &  \textbf{Computer-assisted Implementation}\\\toprule
  \textbf{Categorization}
  & Close reading ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$),
    category identification ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:TextAnalytics}}$, $\S_{\ref{sec:Teaching}}$);
    \emph{taxonomy construction}; \emph{ontology construction}.
  & Distant reading with statistics and statistical graphics ($\S_{\ref{sec:VisGuides}}$);
    cluster and similarity analysis ($\S_{\ref{sec:TextAnalytics}}$);
    text visualization ($\S_{\ref{sec:TextAnalytics}}$);
    \emph{topic modelling};
    \emph{algorithmic taxonomy construction};
    \emph{algorithmic ontology construction}. \\\midrule
  \textbf{Coding}
  & Close reading and labelling ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$); open coding ($\S_{\ref{sec:VisGuides}}$); axial coding ($\S_{\ref{sec:VisGuides}}$); selective coding ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$).
  & Text and discourse analysis ($\S_{\ref{sec:TextAnalytics}}$);
    text visualization ($\S_{\ref{sec:TextAnalytics}}$);
    similarity analysis ($\S_{\ref{sec:TextAnalytics}}$);
    network visualization ($\S_{\ref{sec:TextAnalytics}}$);
    \emph{association analysis}; \emph{ontology mapping}. \\\midrule
  \textbf{Comparative Analysis}
  & Iterative close reading ($\S_{\ref{sec:VisGuides}}$);
    comparing different options of category abstraction ($\S_{\ref{sec:VisGuides}}$);
    continuous refinement of the categorization scheme ($\S_{\ref{sec:VisGuides}}$);
    proposing new categories or categorization schemes ($\S_{\ref{sec:VisGuides}}$). 
  & Iterative and continuous effort for distant reading with statistics and statistical graphics; cluster and similarity analysis; topic modelling; text visualization; algorithmic taxonomy and ontology construction.\\\midrule
  \textbf{Negative Case Analysis}
  & Close reading ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$);
    negative case identification and analysis ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$). 
  & Algorithmic outlier analysis and anomaly detection.\\\midrule
  \textbf{Memoing}
  & Memo-writing ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$);
    sketch-drawing ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$);
    \emph{systematically recording the ideas and actions related to the development of a theory}. 
  & Online discussion forum ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$);
    crowd sourcing ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$);
    provenance visualization ($\S_{\ref{sec:Teaching}}$);
    \emph{data collection from social media}. \\\midrule
  \textbf{Theoretical Sensitivity}
  & Testing a theory against old and new data (i.e., ``Interact'' with data) ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$, $\S_{\ref{sec:EmpiricalStudies}}$);
    analysis of applicability, negative cases, and possible new categories ($\S_{\ref{sec:VisGuides}}$). 
  & Computer-assisted data collection ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$, $\S_{\ref{sec:EmpiricalStudies}}$),
    data analysis and visualization ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:TextAnalytics}}$, $\S_{\ref{sec:Teaching}}$, $\S_{\ref{sec:EmpiricalStudies}}$). \\\midrule
  \textbf{Theoretical Sampling}
  & Data collection ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$, $\S_{\ref{sec:EmpiricalStudies}}$); empirical studies (e.g., controlled experiments ($\S_{\ref{sec:EmpiricalStudies}}$), \emph{surveys, focus groups, field observation, etc.});
  \emph{interview transcription}.
  & Online discussion forum ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$),
    crowd sourcing ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$), and
    \emph{data collection from social media};
    computer-assisted experiments ($\S_{\ref{sec:EmpiricalStudies}}$);
    computer-mediated group activities ($\S_{\ref{sec:Teaching}}$);
    observation of online activities ($\S_{\ref{sec:VisGuides}}$, $\S_{\ref{sec:Teaching}}$). \\\midrule
  \textbf{Theoretical Saturation}
  & \emph{Data collection and analysis until theoretical saturation has been achieved}.
  & Computer-assisted platforms for facilitating the longevity and provenance of the GT processes ($\S_{\ref{sec:VisGuides}}$). \\\bottomrule
  \end{tabular}
  \vspace{-4mm}
\end{table*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/GT/visguides-teaser.pdf}
    \caption{Methodological workflow showing our Grounded Theory approach to the study of visualization guidelines. VisGuides datasets consist of discussions on guidelines and advice in different contexts including education, research, and practice of visualization. Our GT methodological approach is supported by \textit{(i)} computer-supported methods such as text analytics and data visualization, as well as, \textit{(ii)} the collection of empirical data from controlled empirical studies on specific guidelines.}
    \label{fig:teaser}
    \vspace{-4mm}
\end{figure*}


\section{Methodology}
\label{sec:GroundedTheory}
%
%\emph{Grounded theory} (GT) was proposed in the context of the social sciences \cite{Glaser:1967:book}. 

%Consider a postulated theory or a research question (e.g., about social behaviors), 
%% AD: Todo, delete "behavior" replace for another example related to guidelines
%which may be in the form of a categorization scheme, a taxonomy, an ontology, a causal relation, a conceptual model, or a numerical model. GT instigates that the theory needs to be grounded in the data space where the theory emerged, by constantly and continuously sampling the data space, analyzing the data captured, and refining the theory until it reaches theoretical saturation. 


%GT instigates to orient research questions towards \EDIT{explicit facts or instantiations,} what happened (e.g., ``How do people do X?'') rather than \EDIT{requirements or} mental states (e.g., ``What do people want?'' or ``Why do people do X?'' \cite{Willig:2013:book,Strauss:1998:book}.
%We therefore formulated all our six research questions in this work (as described in Section \ref{sec:Introduction}) as ``What happened?'' questions.
%% Rev: R1-16,R2-11, R1-15, R4-6

% \newcommand{\dataset}{$D_{13/03/2019}$}
% \newcommand{\dataset}{\textsc{13/03/2019}}


\subsection{VisGuides}
VisGuides (\url{https://visguides.org/}) is an online discussion forum dedicated to visualization guidelines~\cite{Diehl:2018:EuroVis}.
It allows registered users to pose questions and offer advice on visualization, propose and recommend guidelines, share positive and negative experience about certain guidelines, report and reason about successes, failures, and conflicts of guidelines, and suggest ways to refine guidelines. VisGuides serves us as a digital platform to supply both the \textit{theories}, i.e., the visualization guidelines to be developed and investigated, and the \textit{data}, i.e., the discourses that can be used to generate, evaluate, and refine the theories. Following the tradition in the field of visualization, we use terms such as ``research questions'', ``hypotheses'', ``categorization schemes'', and ``findings'' instead of ``theories'' in the following discussions.

In this paper, we differentiate a \emph{data space} from a \emph{data set}: a data space consists of all possible data sets in a context (e.g., all possible posts that could appear at VisGuides, including those in the future), while a data set is a set of data points as an instance of sampling the data space (e.g., the actual posts in a particular period). VisGuides was launched on September 27, 2017 and on March 13, 2019, when we collected the latest data set \dataset{} for the analysis in this paper, the forum contained 347 posts. The data set \dataset{} contains discourses on prevalent topics in visualization such as color, interaction, virtual reality (VR), and so on. It contains contributions from users with different visualization backgrounds, ranging from undergraduate students to highly-respected visualization experts (e.g., in alphabetic order, Niklas Elmqvist, Stephen Few, Eduard Gr\"{o}ller, Robert Kosara, Liz Marai, Theresa-Marie Rhyne, and Bernice Rogowitz, among others).

\subsection{Methods Outline}

%While we employed traditional GT processes, we also utilized our own expertise in computer-assisted data analysis and visualization to complement the traditional processes. These activities are summarized below, where the same tags used in Table \ref{tab:GroundedTheory}, such as $\S_{\ref{sec:VisGuides}} \backsim \S_{\ref{sec:EmpiricalStudies}}$ and $\S_{\text{A}} \backsim \S_{\text{E}}$, relate the GT processes to individual sections and appendices.

Based on the data collected with VisGuides, we apply the following methods. 

\begin{itemize}[noitemsep, leftmargin=*]

    \item \textbf{Data collection through visualization coursework (Section \ref{sec:Teaching})}: with hundreds of guidelines available in the literature~\cite{kandogan2016grounded}, it would take a very long time for an individual guideline to be investigated or given enough attention. 
    We decided to use VisGuides in our visualization university coursework to achieve both collecting data about guidelines and their usage, as well as to see how the engaging in guidelines discussions could benefit the students. 
    We obtained two data sets from two courses at the University of Swansea $D_{\text{Swansea2019}} \subset \dataset$ and the University of Zurich $D_{\text{UZH2020}}$.
    The close-reading and coding of this two subsets revealed further findings.
    
    \item \textbf{Traditional Categorization and Coding (Section \ref{sec:VisGuides} and Appendix A).}
    The data set \dataset{} collected from VisGuides consists of primarily free text, and supporting images. Thus, any answers to our research questions Q1-Q4 depend critically on the interpretation of this data. According to GT, the key to befitting interpretations is a correct \textbf{categorization} and \textbf{coding}.
    To that end, we close-read all posts in \dataset{} and carried out open and axial coding in order to derive categorization schemes as candidate theories. 
    We used selective coding and statistical graphics to evaluate these categorization schemes. 
    We then propose an integrated categorization scheme to extract information such as ways of mentioning guidelines as well as characteristics of discussions. 
  
    \item \textbf{Text Analysis and Visualization (Section \ref{sec:TextAnalytics} and Appendix C).}
    To complement the traditional approach in Section \ref{sec:VisGuides}, we apply text analysis and text visualization techniques to \dataset, allowing us to observe patterns that could not be derived from close reading easily, such as relationships among keywords mentioned in the text, or the prevalence of some keywords or concepts over other concepts.

    \item \textbf{Empirical Studies (Section \ref{sec:EmpiricalStudies}).}
    To complete our GT-based methodological workflow, we examined two specific guidelines discussed in the forum that indicated a lack of data to backup those guidelines. We conducted two empirical studies to gather more data that could potentially confirm, complete, or contest those exemplary guidelines.
    Such controlled studies are not part of traditional GT but are a common way in Human-Computer Interaction to collect more data besides the traditional text analysis informed by VisGuides. From these controlled user studies, we obtained two additional data sets $E_{\text{KCL2019}}$ and $E_{\text{Konstanz2019}}$. These data sets provide the two guidelines with supporting evidence.
\end{itemize}

% ----------------
% \begin{figure}[t]
%    \centering
%    \includegraphics[height=50mm]{Default}
%    \caption{Caption: Two-way relationship between grounded theory and visualization guidelines. Min}
%    \label{fig:GroundedTheory}
% \end{figure}

==> sections/OldTexFiles/relwork.old.v1.tex <==
\section{Background (0.5-1 page}
\label{sec:RelatedWork}

\ben{Ben to draft.  All to contribute references.}

%%%%%
\subsection{What are guidelines?}

Guidelines have been defined as \textit{a general rule, principle, or piece of advice}~\cite{guidelineoxford} and \textit{information intended to advise people on how something should be done or what something should be}~\cite{guidelinecambridge}. Thus, guidelines serve as guardrails for good practices and to help avoiding pitfalls. Guidelines are practical, focused on action, and possibly lend themselves to a mathematical formalization, e.g., \textit{do X, avoid Y}~\cite{Chen:2017:CGA}. A collection of such related guidelines (e.g., on the topic of using colors in visualization) can inform the development of a conceptual model~\cite{Chen:2017:CGA} (e.g., about color perception in visualization) such as Bertin's visual variables~\cite{bertin1983} or Mackinlay's research on performance for specific data types~\cite{Mackinlay_1986}. 

At the same time, guidelines are never mandatory. Rather, they usually are limited as many of them focus on specific cases. Guidelines even can even contradict each other. Our works aims in surfacing and presenting guidelines in visualization as well as to suggest a way of collecting and analyzing guidelines for visualization

%A recent workshop identified  
%'principles and guidelines' as one of four aspects of theoretical advances in visualization, alongside 'taxonomies and ontologies', 'conceptual models and theories frameworks', 'laws and theoretic systems'~\cite{Chen:2017:CGA}. Or example, Bertin's visual variables~\cite{bertin1983} or  Mackinlay's research on performance for specific data types~\cite{Mackinlay_1986} are higher-level frameworks.

% However, while these theories have huge and well acknowledged practical implications, they do not \textit{prescribe} any specific action for a given case. 
% Guidelines, on the other side, have a prescriptive character, have direct practical implications and help making decisions. 

%%%%%
\subsection{Visualization Guidelines}

Guidelines in visualization (\textit{visualization guidelines}) have been part of the evolution of the visualization discipline since its beginning, with contributions from visual arts, perception, and psychology. Prominent examples of visualization guidelines include 
Sheiderman's Mantra \textit{Overview first, zoom and filter, details on demand}~\cite{shneiderman2003eyes}, 
\textit{`Colormap considered harmful'}~\cite{}, 
\textit{Create the simplest graph that conveys the information you want to convey}~\cite{tufte2001visual}, or 
\textit{Select meaningful axis ranges}~\cite{robbins2012creating}. A range of guidelines can be found in papers that propose guidelines as lessons learned for a particular subject, often resulting from empirical quantitative studies or application case studies. Visualization guidelines can be found for text 
highlighting techniques~\cite{strobelt2016guidelines}, 
the use of multiple views~\cite{wang2000guidelines},
hierarchical visualizations~\cite{elmqvist2010hierarchical}, 
the design of information visualization applications~\cite{carr1999guidelines}, 
the design of charts for publication~\cite{kelleher2011ten}, 
making visualizations memorable~\cite{borkin2016beyond}, 
avoid deception~\cite{jones2011lie,monmonier2018lie}, 
use of embellishment in charts~\cite{bateman2010useful},
for visual analytics~\cite{perer2009integrating}, 
for the use of color~\cite{brewer1994color,brewer1994guidelines,borland2007rainbow,silva2011using} and many more.
\ben{more of these examples here?}

However, there is little previous works that proposes and structures a general overview of guidelines. Examples of guideline collections and surveys include Silva's et al. \cite{silva2011using} collection of  guidelines for the use of color in information visualization;
Brodbeck et al. \cite{brodbeck2009interactive} design guidelines for interactive visualizations; and 
Borgo et al. \cite{borgo2013glyph} guidelines for glyph-based visualizations. 

%Many more guidelines can be found online in a rich set of websites, blogs~\cite{DosandDonts,topten,sixguidelines} . However, many of these 'open' guidelines did not underwent scientific peer-reviewing and might lack references and validation. Moreover, as guidelines are always limited and may be valid only for specific cases, we need a better framework for collecting, communicating, and discussing guidelines~\cite{engelke2018visupply}. 
%%%%%
\subsection{Collecting, Curating, and defining guidelines}

Collection, storage, and definition of guidelines are currently not centrally organized. While many guidelines originate and are written down in from scientific papers based on empirical studies, application case studies, or surveys (see above), others originate from blogs or class-room material such as slides~\cite{DosandDonts,topten,sixguidelines}. Fora are sometimes used to discuss guidelines (for an extensive list or fora see~\cite{engelke2018visupply}). Across these media, Scott-Brown~\cite{Scott-Brown2018Presenting} found guidelines reported as \textit{text}, visual, or automated \textit{decision trees}~\cite{data-to-viz}, \textit{checklists}~\cite{datavischecklist} or design patterns~\cite{bach2018narrative,bach2018design}. Eventually, guidelines could be implemented in the form of concise cheat sheets~\cite{WhichVisualization,betterpresentations}. A comprehensive summary of ``about 550 guidelines'' is provided by Kandogan et al.~\cite{Kandogan_2016}, extracted from books, papers, and blogs. The authors compiled statistical summaries of the guidelines and constructed a three-level hierarchy of concepts, sub-concepts and instances using a grounded theory analysis of guidelines, defining a total of 515 categories such as concepts data, visualization, 
users, insights (including tasks supported and knowledge gained), device (physical aspect of visualization medium), and qualifiers indicating specific qualities and quantities in a guideline.

More structured approaches can be found in medicine, where repositories for guidelines exist that capture about 6000 guidelines~\cite{guidelinesinternational}, while the PLOS and Nature journals feature short summary article tracks including data visualization~\cite{naturemethods,plostensimplerules}. Similarly, Scott-Brown suggests a formal and central storage to visualization, alongside with a unique ID, tags, categories, and relations to other guidelines. To streamline the live-cycle of guidelines, Engelke et al. propose a framework for the curation, discussion, and communication of visualization guidelines~\cite{engelke2018visupply} and which consists of steps such as \textit{collection}, \textit{integration}, \textit{contextualization}, \textit{generalization}, and \textit{guideline definition}. 

%As articulated in \cite{Chen:2017:CGA}, visualization guidelines can provide the taxonomies and ontologies in visualization with keywords and causal relations.
%Each guideline can be mapped to a mathematical conjecture, and it can potentially become a theorem when it is mathematically confirmed.
%A collection of related guidelines (e.g., on the topic of using colors in visualization) can inform the development of a conceptual model (e.g., about color perception in visualization).
Our goal is to present methods to obtain a representative picture of the current landscape of guidelines, to rank the most popular ones in the visualization field, and to obtain insights into how to structure and create `guidelines for guidelines'. For example, a guideline may come in a variety of different formats; it can be stated as an imperative (e.g., xx~\cite{}), a suggestion (e.g., ), a fact or pointer to a piece of empirical knowledge (e.g., \textit{humans can only discriminate around 7 colors}). By openly coding replies in our forum, we are interested in how people express and formalize visualization in general and visualization guidelines in particular. 
We also report on the popularity of guidelines weighting citations, subjective expert reporting, trustworthiness of the resources, among other indicators.

\ben{complete}.

\newpage

==> sections/OldTexFiles/relwork.tex <==
% --------------------
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/GT/GT-VisGuides.pdf}
    \caption{Caption}
    \label{fig:GTandVisGuides}
\end{figure*}
% --------------------

\section{Background}
\label{sec:RelatedWork}

\subsection{Guidelines in Visualization}
\label{sec:BG-Guidelines}
%
A guideline is a \textit{``general rule, principle, or piece of advice''} \cite{guidelineoxford} that provides \textit{``information intended to advise people on how something should be done or what something should be''}~\cite{guidelinecambridge}. In the area of information visualization, guidelines can be used as heuristics for evaluation~\cite{Zuk:2006:BELIV} or to help practitioners make choices in developing visual designs and visualization systems~\cite{Meyer:2015:IV}. 
%In this paper, we extend the use of guidelines to active discussion by using an online forum. 

Many surveys have collected guidelines, including general rules on how to use colors in information visualization \cite{silva2011using}, design guidelines for certain properties of visualizations, such as interactive visualizations \cite{brodbeck2009interactive}, visualization in scientific publications \cite{kelleher2011ten}, and design patterns for storytelling~\cite{bach2018narrative,bach2018design}; but also for certain types of visualizations, such as glyph-based visualizations \cite{borgo2013glyph}. A good number of these guidelines are known to visualization researchers and practitioners, such as \textit{``the rainbow color map is harmful''} \cite{Rogowitz:1998:S,Borland:2007} and \textit{``maximize data-ink ratio''} \cite{tufte2001visual}. Some of these guidelines have been widely endorsed such as, for example, Ben Shneiderman's \textit{``overview first, zoom and filter, then details-on-demand''} \cite{Shneiderman:1996:VL}. The ``zoom'' part has been mathematically proven~\cite{Chen:2010:TVCG} and it was the discoveries of the occasional preference in some applications for ``details first'' \cite{vanHam:2009:TVCG,Luciani:2019:TVCG} that led to better understanding of its underlying rationale~\cite{Chen:2016:book}. 

Chen et al. asserted that guidelines are an integral part of the theoretical foundation of visualization and instigated the need for curating, evaluating, critiquing, and refining guidelines in an open and transparent manner, including the adoption of GT~\cite{Chen:2017:CGA}. While some guidelines are explicitly stated as such, e.g., in text books~\cite{tufte2001visual} or research papers~\cite{bateman2010useful}, many guidelines may not be explicitly phrased as guidelines but can be extracted from research findings, theoretical propositions, and experience from design applications. For example, Bertin's findings on the suitability of different retinal variables (visual channels) for four types of perception~\cite{Bertin:1983:book} can easily be rephrased as ``do'' and ``don't'' statements. The use of such for guideline construction, for example ``do'' and ``don't'', raises questions about how to formalize, present, disseminate, and discuss guidelines within as well as \textit{beyond} the core visualization community. For example, Engelke et al.~proposed a supply chain framework for the life-cycle of guidelines, formalizing the process of generating, confirming and updating guidelines~\cite{engelke2018visupply}, and Scott-Brown discussed ways for presenting collections of guidelines in a structured and uniform manner~\cite{Scott-Brown2018Presenting}. % \ben{more detail}. \alex{maybe we change or remove part of this text}

Previous work has focused on data collection and analysis of taxonomies and ontologies of guidelines. A first study by Kandogan and Lee~\cite{kandogan2016grounded} identified 550 visualization guidelines and found that they ranged between 5 to 140 words. While such work is helpful in finding and recording guidelines, we require better data to understand how people use, formulate, and discuss guidelines as well as how guidelines can become a widely accepted tool for visualization research (e.g., How to inform hypotheses from guidelines or Which guidelines can be used as a basis for research hypotheses?), teaching (e.g., Which guidelines are agreed-upon? How to apply and dispute guidelines in an educational context?), and application (e.g., Which guidelines are relevant for a specific problem? How to make trade-offs? How to use guidelines for evaluation?).


\subsection{Grounded Theory}
\label{sec:BG-GT}
%
Grounded Theory (GT) is a research methodology centered at the principle that theories must be grounded in the data%
\footnote{GT itself is not a theory. In this paper, the term ``a theory'' means a theoretical postulation that is to be formulated and evaluated using GT methods, unless it is stated explicitly as a confirmed theory.}.
GT was first proposed by Glaser and Strauss for sociological research \cite{Glaser:1967:book} with the goal of constructing and scrutinizing theories from data. Applying GT includes 
\textit{(1)} collecting data, e.g., in the form of examples, counter examples, and case studies. Subsequently, 
\textit{(2)} these data can stipulate techniques and processes for grounding theories through methods such as as \emph{categorization}, \emph{coding}, \emph{constant comparative analysis}, \emph{negative case analysis}, \emph{memoing} (see summary in Table~\ref{tab:GroundedTheory}). The formal descriptions of these methods and principles, which was compiled based on the work of Willig~\cite{Willig:2013:book}, can be found in Appendix D. The ultimate goal of GT is to scrutinize the theory by constantly and continuously sampling the data space, analyzing the data captured, and refining the theory until it reaches \emph{theoretical saturation}.

As illustrated in Fig. \ref{fig:GTandVisGuides}, the scope of GT has been broadened over the past five decades \cite{Kenny:2014:QR}.
The original version of GT asserted that a theory must be ``naturally'' emerged from the data, and GT researchers must be open-minded and must abstain from existing theories in the literature.
1990 saw the first major extension of the scope.
Strauss (one of the original proposers) and Corbin challenged this assertion, reinterpreting ``open mind'' as not ``empty mind'' \cite{Strauss:1990:book}.
This broadened the scope of GT beyond the restriction of studying ``naturally-emerged'' theories only.
In 2006, Charmaz, a student of Strauss and Glaser, further broadened the scope of GT by allowing GT researchers to use their prior knowledge more actively, especially in coding, sampling, raising question, and determining the focuses of further iterations \cite{Charmaz:2006:book}.
Meanwhile, Glaser argued to preserve the original scope of GT, which is now referred to as \emph{Classic GT}, while the two extended versions are referred to as \emph{Straussian GT} and \emph{Constructivist GT} respectively. 
The insistence for maintaining the ``pure GT'' is sometimes referred to as \emph{Glaserian GT}.

Several other extensions were proposed before or around 2010.
The SAGE Handbook of Grounded Theory edited by Bryant and Charmaz \cite{Bryant:2010:book} consists of 27 articles on GT, featuring different versions and applications of GT.
In their introductory article of the handbook \cite{Bryant:2010:bookCh1}, Bryant and Charmaz explicitly defined ``grounded theory method as a family of methods,'' and marked the handbook as a celebration of difference.
In another article, Denzin identified seven versions of GT, positivist, postpositivist, constructivist, objectivist, postmodern, situational, and computer assisted GT \cite{Denzin:2010:bookCh21}, with the first three roughly corresponding to the aforementioned classic GT and its two extensions.

In their introductory chapter \cite{Bryant:2010:bookCh1}, Bryant and Charmaz also noted that the original GT did not in anyway reject quantitative methods.
Glaser and Strauss ``intended to show such [qualitative] research projects could produce outcomes of equal significance to those produced by the predominant statistical-quantitative, primarily mass survey methods of the day.'' ``Glaser has always argued that the method applies equally to quantitative inquiry.''
In fact, Glaser and Strauss clearly stated in their 1967 book \cite{Glaser:1967:book}:%
\footnote{The italicized excerpts were highlighted by Glaser and Strauss originally in their book\cite{Glaser:1967:book}.}
``Our position in this book is as follows: there is no fundamental clash between the purposes and capacities of qualitative and quantitative methods or data. ... We believe that \emph{each form of data is useful for both verification and generation of theory,} whatever the primacy of emphasis. ... \emph{In many instances, both forms of data are necessary}.''
Many scholars have adopted mixed-methods approaches featuring both qualitative and quantitative methods.
For example, Brannen included GT as a major method in her 1995 book on mixed methods \cite{Brannen:1995:book}. 
Almost all books thereafter on mixed methods approaches have included GT as component method (e.g., \cite{Creswell:2002:book,Todd:2004:book,Bergin:2018:book}).
In 2010, Johnson et al. proposed a mixed-methods version of GT (MM-GT) for ``connecting theory generation with theory testing'' \cite{Johnson:2010:RiS}.

The contemporary, broadened scope of GT provides an ideal research framework for applying qualitative research methods to the discourse data accumulated at VisGuides, while the GT-based studies can benefit from the research methods familiar to visualization researchers, such as digital data collection, text visualization, and empirical studies).

\subsection{Grounded Theory for Visualization Guidelines}
\label{sec:BG-GT4VisGuides}
%
In the context of visualization guidelines, one may collect raw data about all (a) statements of, (b) discourses on, (c) scientific studies on, and (d) application case studies of visualization guidelines.
For (a), the corpus of 550 guidelines by Kandogan and Lee~\cite{kandogan2016grounded} is the largest collection reported so far.
VisGuides focuses on (b), while stimulating new efforts for creating a public corpus of (a) and conducting surveys of (c) and (d).

Once there is such raw data, GT methods can be applied to the data to discover new theories.
In their GT study on the language characteristics of visualization guidelines~\cite{kandogan2016grounded}, Kandogan and Lee used coding to identify five high-level concepts in guidelines (\textit{Data}, \textit{Visualization}, \textit{User}, \textit{Insight}, and \textit{Device}) as well as a refining/contextualizing the concept (\textit{Qualifier}) that a guideline may feature.
This provides an important step towards the goal of GT, i.e., to discover and evaluate theoretical hypotheses by exploring the relationships among these concepts \cite{Glaser:1967:book}.

Similarly, if VisGuides can provide a corpus of (b), one can use GT methods to first identify core categories and properties through coding and obtain their statistical measures (indices in \cite{Glaser:1967:book}).
One can then gradually progress towards hypothesis discovery and evaluation.
As shown in Fig. \ref{fig:GroundedTheory}, this is the first GT application to be reported in this work.
Similar to~\cite{kandogan2016grounded}, we have completed a coding exercise but are yet to report any discovered hypotheses.

As observed in \cite{Chen:2017:CGA}, each visualization guideline defines a causal relation and is thus a hypothesized theory. Because most visualization guidelines are not discovered using GT methods, the original GT distanced itself from studying such theories.
The extensions made in Straussian GT and Constructivist GT have provided a mandate for us to study individual visualization guidelines as hypothesized theories using GT methods.
This is the second GT application to be reported in this work.

The concept of Situational GT was first proposed by Clarke in 2003 \cite{Clarke:2003:SI} and was recognized as an extension of GT some years later \cite{Denzin:2010:bookCh21}.
It advocated ``discourses are analytical modes of ordering the chaos of the world,'' and the need for studying human subjects as well as ``non-human objects in situations -- things of all kinds.'' It outlined a GT method for making three kinds of maps through analyzing data and memos: situational maps, social worlds/arenas maps, and positional maps \cite{Clarke:2007:book}.
This inspires to study visualization guidelines in education as a specific situation, resulting in third GT application to be reported in this work.

When proposing the classic GT \cite{Glaser:1967:book} in 1967, Glaser and Strauss stated: ``It must be remembered that qualitative data suggesting a category may also be used as another slice of data for the quantitative analysis.'' They included statistical measures (referred to as indices) in five tables in their book. If text visualization techniques were available at that time, Glaser and Strauss might include such techniques as GT tools. by 2010, computer-assisted GT was considered as a GT extension \cite{Denzin:2010:bookCh21}. In the SAGE Handbook of Grounded Theory \cite{Bryant:2010:book}, the word ``computer'' appeared in some 50 places in the context of aiding GT. The book also included a hand-drawn network visualization of different categories resulting from coding.
These all indicate that using visualization techniques to aid GT is not a violation of GT principle.
In this work, we use text analysis to aid the first and second GT applications.

In their 1967 book \cite{Glaser:1967:book}, Glaser and Strauss also discussed statistical sampling and control variables. They acknowledged that ``when the sociologist wishes also to describe the magnitude of relationship within a
particular group, random sampling, or a highly systematic
observation procedure done over a specified time is necessary.''
However, they did argue: ``Statistical tests of significance of an association between variables are not necessary'' because they ``present a strong barrier to the generation of theory''. 
In 2010, Johnson et al. built on Glazer and Strauss's view that GT worked well with both qualitative and quantitative data, outlined the scope of MM-GT \cite{Johnson:2010:RiS}.
Hence, this enables us to use controlled experiments to support the second GT application and test some visualization guidelines within the scope of MM-GT.

-----------------------------------\\
The following texts are to be moved around.\\
-----------------------------------\\

%Recently, Bradley et al. suggested that visualization research can benefit from a range of research methods in humanities and social science (including GT) \cite{Bradley:2018:CGA}.

 %% very confusing.
Our work in this paper follows this general research agenda on visualization guidelines envisaged by these works and adds more empirical evidence towards an emerging \textit{theory of guidelines}.

In addition to considering visualization guidelines as individual theories, we can anticipate the possibility of formulating meta-theories that model different aspects of the corpus of visualization guidelines, e.g., their categorization \cite{kandogan2016grounded} and their life-cycle \cite{engelke2018visupply}. According to GT, such meta-theories should also be grounded on the relevant data, which may include different expressions of the guidelines, the attributes of each expression (e.g., originator, location, period, context, etc.), and documentation about their formulation, discussion, curation, sharing, application, evaluation, refinement, and so on. 
In our paper, we propose a categorization scheme that consequently captures data about \textit{how people understand and discuss guidelines} and give advice, rather than (just) \textit{enumerating guidelines}. As detailed in Section~\ref{sec:GroundedTheory}.
The explicit formulation of guidelines can be part of how people communicate advice. 

Our approach goes beyond the formulation of guidelines and seeks for formal theory of guidelines and an structured method to obtain appropriate data for such a theory.
We are the first to propose a methodological approach for visualization guidelines based on the traditional set of GT methods, detailed in Fig.~\ref{fig:GT-overview}, by 
\textit{(i)} computer-supported methods such as an online-forum, text analysis, data visualization, as well as 
\textit{(ii)}, the collection of empirical data from empirical subject-matter studies about specific guidelines. These approaches provide us with a far greater variety and quality of of data.


%A recent workshop identified  
%'principles and guidelines' as one of four aspects of theoretical advances in visualization, alongside 'taxonomies and ontologies', 'conceptual models and theories frameworks', 'laws and theoretic systems'~\cite{Chen:2017:CGA}. Or example, Bertin's visual variables~\cite{bertin1983} or  Mackinlay's research on performance for specific data types~\cite{Mackinlay_1986} are higher-level frameworks.

% However, while these theories have huge and well acknowledged practical implications, they do not \textit{prescribe} any specific action for a given case. 
% Guidelines, on the other side, have a prescriptive character, have direct practical implications and help making decisions. 

%%%%%
% \textcolor{red}{Plan to remove the paragraph below.}

% Guidelines in visualization (\textit{visualization guidelines}) have been part of the evolution of the visualization discipline since its beginning, with contributions from visual arts, perception, and psychology. Prominent examples of visualization guidelines include 
%\textit{Create the simplest graph that conveys the information you want to convey}~\cite{tufte2001visual}, or 
%\textit{Select meaningful axis ranges}~\cite{robbins2012creating}. A range of guidelines can be found in papers that propose guidelines as lessons learned for a particular subject, often resulting from empirical quantitative studies or application case studies. Visualization guidelines can be found for text 
% highlighting techniques~\cite{strobelt2016guidelines}, 
% the use of multiple views~\cite{wang2000guidelines},
% hierarchical visualizations~\cite{elmqvist2010hierarchical}, 
% the design of information visualization applications~\cite{carr1999guidelines}, 
%the design of charts for publication~\cite{kelleher2011ten}, 
% making visualizations memorable~\cite{borkin2016beyond}, 
% avoid deception~\cite{jones2011lie,monmonier2018lie}, 
% use of embellishment in charts~\cite{bateman2010useful},
% for visual analytics~\cite{perer2009integrating}, 
% for the use of color~\cite{brewer1994color,brewer1994guidelines,borland2007rainbow,silva2011using} and many more.


%Many more guidelines can be found online in a rich set of websites, blogs~\cite{DosandDonts,topten,sixguidelines} . However, many of these 'open' guidelines did not underwent scientific peer-reviewing and might lack references and validation. Moreover, as guidelines are always limited and may be valid only for specific cases, we need a better framework for collecting, communicating, and discussing guidelines~\cite{engelke2018visupply}. 
%%%%%

% Collection, storage, and definition of guidelines are currently not centrally organized. While many guidelines originate and are written down in from scientific papers based on empirical studies, application case studies, or surveys (see above), others originate from blogs or class-room material such as slides~\cite{DosandDonts,topten,sixguidelines}. Fora are sometimes used to discuss guidelines (for an extensive list or fora see~\cite{engelke2018visupply}). Across these media, Scott-Brown~\cite{Scott-Brown2018Presenting} found guidelines reported as \textit{text}, visual, or automated \textit{decision trees}~\cite{data-to-viz}, \textit{checklists}~\cite{datavischecklist} or design patterns~\cite{bach2018narrative,bach2018design}. Eventually, guidelines could be implemented in the form of concise cheat sheets~\cite{WhichVisualization,betterpresentations}.

\subsection{Previous Applications of GT in Visualization}
%
In addition to the aforementioned work on visualization guidelines by Kandogan and Lee~\cite{kandogan2016grounded}, the visualization community has used GT in many other applications.
Coding, one of the key process in GT, has been widely used for categorizing raw data in the context of visualization and HCI.%
\footnote{Strictly speaking, as a qualitative data analysis method, coding was invented before the emergence of GT.
In their 1967 book, Glaser and Strauss cited Udy's 1964 comment \cite{Udy:1964:book}: ``The coding operation proved to be very tedious `dog work' in the worst sense of the term.'' Nevertheless, GT has introduced several coding methods and developed coding into a systematic practice in qualitative research.}
\alex{For example, Sprague and Tory~\cite{Sprague:2012:IV} used GT guidelines for coding their interviews, images, and sketches to analyze key promoting and inhibiting factors in the use of visualization in casual contexts. They generate ad hoc tag names using theoretical coding to help identify commonalities between topics.
% --> No comparative analysis mentioned
%Borgo et al. used coding to do ?X? ~\cite{borgo2018information}.
Hullman and Bach~\cite{hullman2018picturing} used an open coding approach to categorize graphical abstracts and their different level of abstraction and the way they employ visual and spatial structures, text, and other graphical entities.
McKenna et al.~\cite{mckenna2015unlocking} used open coding to cognitive task analysis papers to understand the cognitive activities of users. 
Isenberg et al.~\cite{isenberg2016visualization} used a multi-pass manual coding combined with automatic clustering, re-fining of the topic
clusters and comparative analysis.
Lam et al.~\cite{lam2017bridging} used coding to categorize and structure design study papers into specific goals and abstract tasks.
Waldner et al.~\cite{waldner2019comparison} used coding of crowdsourced data to compare two different visual designs.
Blascheck et al.~\cite{blascheck2018exploration} coded eye-tracking
visualizations, video, and audio recordings
to identify exploration strategies and behavior of user visual interactions.
}
%\textbf{There are more coding papers.}

\textbf{Did any paper managed to come out a theoretical hypothesis after coding? Are there any GT papers other than coding? }
In addition, Chandrasegaran et al. proposed to use visual analytics to aid GT processes with a case study of a qualitative text analysis~\cite{Chandrasegaran:2017:CGF}.
\alex{Blascheck et al.~\cite{blascheck2016visual} also proposed a visual analytics framework for facilitating interactive coding of user behavior.
Drouhard et al.~\cite{drouhard2017aeonium} presented a visual analytics interface that supports collaborative coding and allows for the continues analysis and refinement of the qualitative coding.}

%% Alex
%% although these previous....xxxx



% responses from interviews, visualization techniques, evaluation methods, picture elements~\cite{hullman2018picturing}, and many other things. From the perspective of GT, most visualization guidelines are theories since almost all these guidelines were proposed based on the originators' observation and experience, or on the results of empirical studies. GT instigates to orient research questions towards evidence about what \textit{happened} (e.g., How do people do X?) rather than requirements or  \textit{mental states} (e.g., What do people want? Why do people do

%Kandogan et al.~\FIXME{~\cite{kandogan2016grounded} in their study on the language characteristics of visualization guides identified five high-level concepts in guidelines (\textit{Data}, \textit{Visualization}, \textit{User}, \textit{Insight}, and \textit{Device}) as well as a refining/contextualizing concept (\textit{Qualifier}) that a guideline may feature. \alex{Using open coding and axial coding, which are part of GT,} they further identified categories to characterize language features in guidelines for conveying relationships between high-level concepts and considered language forms for conveying \textit{instructions}, \textit{conditions}, \textit{rankings}, and \textit{explanations}.} As the data used in that study is not publicly available, it is not easy to build further on it using GT or any other method. In comparison to our work, Kandogan et al.~focused on the \textit{open} discourse of guidelines and their uses in practical scenarios. \FIXME{Our analysis has to be seen in the specific context of a deliberate data collection process through an online forum and teaching activities shifting the focus to a much more active, explicit, and indirect engagement with guidelines rather than gathering guidelines from their direct sources as done by Kandogan et al.} 



% GT is not limited to guidelines but can be applied to unite and verify a broader set of theoretical frameworks such as taxonomies, ontologies, and conceptual models.


% The Human-Computer Interaction (HCI) and Visualization communities have applied GT in the form of \textit{coding}, e.g., responses from interviews, visualization techniques, evaluation methods~\cite{borgo2018information}, picture elements~\cite{hullman2018picturing}, and many other things. From the perspective of GT, most visualization guidelines are theories since almost all these guidelines were proposed based on the originators' observation and experience, or on the results of empirical studies. GT instigates to orient research questions towards evidence about what \textit{happened} (e.g., How do people do X?) rather than requirements or  \textit{mental states} (e.g., What do people want? Why do people do X?)\cite{Willig:2013:book,Strauss:1998:book}. Moreover, we argue that a visualization guideline should be considered as a postulated theory in the form \textit{A leads to B} (sometimes amended through a \textit{condition C}); e.g., `Rainbowmaps (\textit{A}) are considered harmful (\textit{B})'.
% Eventually, the goal is to map such a formalization to a mathematical conjecture (e.g., \texttt{A$\Rightarrow$B}, under condition \texttt{C}), which can potentially become a theorem when it is mathematically confirmed. Analyzing our forum (see Section~\ref{sec:VisGuides}) provides us with a first idea of how people understand, discuss, and critically object guidelines, in which other forms do people give advice, and which evidence (if any) is provided. Text analysis (Section \ref{sec:TextAnalytics}) provides a distant-reading approach to understand groups and hierarchies among topics mentioned in the forum and controlled user studies in Section \ref{sec:EmpiricalStudies} add further quantitative data to assess the strength and validity for a given guideline conjecture.




==> sections/OldTexFiles/table-H1H2.tex <==
\begin{table*}[t]
  \caption{The categories of the variable \textbf{H1: Main Purpose}.}
  \label{tab:H1}
  \centering
  \begin{tabular}{@{}p{2.5cm}@{\hspace{2mm}}p{15cm}@{}}
    \toprule
    \textbf{Variable} & \textbf{Definition and Explanation}\\
    \midrule
    \textbf{H1. Main Purpose} &
    The main purpose of the post (related to ``Purpose'' in RST). The post exhibits more than one purpose, the coder will make a judgment about what the main one is.\\
    \midrule
    \textbf{Category} & \textbf{Definition and Explanation}\\
    \midrule
    \emph{Ask for Advice} &
    A post asks for information about some techniques, guidelines, theories, etc. This includes posts for seeking advice on specific problems, but does not includes posts for seeking clarification from the author of a previous post, nor posts for challenging or critiquing through an expressive question.\\ 
    \emph{Offer Advice} &
    A post that is intended to offer advice, and to pass on knowledge and experience for helping others who are seeking advice. This includes posts that volunteer the author's or someone's guidelines without any prompt, as well as posts that were intended to offer alternative advice that may differ from or in conflict with the advice given by others.\\
    \emph{Discuss Guidelines} &
    A post that focuses on guidelines, it may question the correctness of a guideline or an aspect of a guideline, comment on a guideline, critique guideline, or defend a guideline. This category does not include offering references about guideline, explaining a guideline, or providing advice involving a guideline.\\
    \emph{Seek Clarification} &
    A post seeks a clarification from the author of a previous post that could be asking a question or offering some advice, information, or comment. For example, one may ask ``when you say a colormap, do you mean a continuous or discrete colormap?''\\
    \emph{Add Clarification} &
    A post provides a clarification about some statements in a previous post. To distinguish this from ``ask advice'', ``offer advice'', or ``discuss guideline'', the emphasis is the additionality to the previous post. If the post contains a substantial amount of new information, it is better to use one of the other categories.\\
    \emph{Social Conversation} &
    Acknowledgement, etiquette, or any social conversation, such as ``Thank you.''\\
    \emph{Administration} &
    This is reserved for any administrative posts sent by VisGuides managers.\\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{The categories of the variable \textbf{H2. Guideline Mentioning}.}
  \label{tab:H2}
  \centering
  \begin{tabular}{@{}p{3.8cm}@{\hspace{2mm}}p{13.7cm}@{}}
    \toprule
    \textbf{Variable} & \textbf{Definition and Explanation}\\
    \midrule
    \textbf{H2. Guideline Mentioning} &
    The way in which guidelines are mentioned in the post (``Claim'' and ``Support'' in RST).\\
    \midrule
    \textbf{Category} & \textbf{Definition and Explanation}\\
    \midrule
    \emph{Direct} &
    Mentioning a guideline explicitly, such as according to X, ``one should do this''. If someone proposes a NEW guideline himself or herself, it belongs to this category.\\
    \emph{Indirect} &
    Mentioning a reference to a publication, a blog, but without spelling out a guideline,     e.g., ``there is a fact about color [REF], thus it is better to do this.''\\
    \emph{Implicit} &
    Referring to a reasonably well-known guideline but without mentioning it clearly. For example, ``you may consider maximizing data-ink ratio here''. To select this category, the coder must add a link or reference in the comment section.\\
    \emph{Unclear or Possible} &
    The coder suspects that there might be an implicitly mentioned guideline, but cannot determine any reference or source.\\
    \emph{None} &
    The coder cannot identify any guideline mentioned in the post, and is reasonably sure that no guideline was mentioned in the post.\\
    \bottomrule
  \end{tabular}
\end{table*}

==> sections/OldTexFiles/table-H3H4.tex <==
\begin{table*}[t]
  \caption{The categories of the variable \textbf{H3. Evidence}.}
  \label{tab:H3}
  \centering
  \begin{tabular}{@{}p{2.5cm}@{\hspace{2mm}}p{15cm}@{}}
    \toprule
    \textbf{Variable} & \textbf{Definition and Explanation}\\
    \midrule
    \textbf{H3. Evidence} &
    The level of details of the evidence the post provides to support something (a technique, a visual design, a guideline, etc.) works, does not work, or needs to be addressed (related to ``Evidence'' and ``Elaboration'' in RST).\\
    \midrule
    \textbf{Category} & \textbf{Definition and Explanation}\\
    \midrule
    \emph{Detailed} &
    One or more examples or case studies are clearly given such as in many posts by Swansea students. There is little imagination required by a reader to understand the evidence.\\
    \emph{Brief} &
    A short description (typically one sentence, one or two references) that a reader has to imagine the actual scenario, or go read the reference. For example, ``this is similar to the technique that worked for bio-visualization.''\\
    \emph{Unclear} &
    The coder suspects that some statements in the post may imply some evidence, but cannot be sure about this.\\
    \emph{None} &
    The coder cannot identify any evidence mentioned in the post, and is reasonably certain that the post does not include any evidence.\\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{The categories of the variable \textbf{H4. Main Scope}.}
  \label{tab:H4}
  \centering
  \begin{tabular}{@{}p{2.5cm}@{\hspace{2mm}}p{15cm}@{}}
    \toprule
    \textbf{Variable} & \textbf{Definition and Explanation}\\
    \midrule
    \textbf{H4. Main Scope} &
    The scope that the post covers or intends to cover (related to ``Circumstance'' and ``Condition'' in RST). When a post has different types of coverage, the coder will make a judgment as the main coverage intended for this post. For example, if a post focuses on advising a specific design of an interaction, suggesting ``you should use `radio buttons' for this interaction, though I prefer check boxes in general,'' one may consider this to be a case-based scenario.\\
    \midrule
    \textbf{Category} & \textbf{Definition and Explanation}\\
    \midrule
    \emph{Case-based} &
    The post focuses on one or more individual cases, such as the problems related to a specific data set or visual design in most posts by Swansea students.\\
    \emph{Conditional} &
    This post focuses on a good number of cases that may fall under certain conditions. Here condition is defined as a smaller scope than context. Examples include ``can parallel coordinates deal with more than 100 axes?'', ``how can one design a multivariate bar charts without using colors?'', and ``this guideline does work in most situations, but not in the following conditions.''\\
    \emph{Contextual} &
    This post focuses on a specific context that can easily cover many example cases. The contexts may be defined at a relatively high-level, such as topics (e.g., interaction, color), visual representations (bar charts), users (e.g., domain experts), tasks (navigation), applications (e.g., sports), and so on.\\
    \emph{General} &
    The post focuses on a very general discussion about the field of visualization or beyond such as computer science, data science.\\
    \emph{Unclear} &
    The coder detects some focal topics in the post, but cannot be certain about its scope.\\
    \emph{No Focal Topic} &
    The coder is reasonably sure that this post does not have a focal topic. This includes those posts for acknowledgement, and social conversation.\\
    \bottomrule
  \end{tabular}
\end{table*}

==> sections/OldTexFiles/table-H5H6.tex <==
\begin{table*}[t]
  \caption{The categories of the variable \textbf{H5. Antithesis}.}
  \label{tab:H5}
  \centering
  \begin{tabular}{@{}p{2.5cm}@{\hspace{2mm}}p{15cm}@{}}
    \toprule
    \textbf{Variable} & \textbf{Definition and Explanation}\\
    \midrule
    \textbf{H5. Antithesis} &
    The Level of Agreement with previous posts, excluding any future posts (related to ``Antithesis'' in RST). The categories are defined in relation with all previous posts in the thread. It is not about agreement with a particular guideline, opinion, or advice, which will not be easy to code without specifying which guideline, opinion, or advice.\\
    \midrule
    \textbf{Category} & \textbf{Definition and Explanation}\\
    \midrule
    \emph{Neutral} &
    The post does not show any opinion that could possibly be in disagreement with previous post. This includes typical posts for seeking information or advice. However, it does not include posts that challenge or question existing guidelines.\\
    \emph{So Far So Good} &
    The post has an opinion, poses a challenge to a guideline, or offer an advice, but it has not yet in disagreement with previous posts (implying all previous posts are in agreement). This includes the first post for opening a thread with a comment or question that challenges a guideline. \\
    \emph{Objection} &
    The post has at least one opinion that disagrees with some opinions in the previous posts. This includes posts for defending one's own opinions after being criticized.\\
    \emph{Unclear} &
    The coder detects some opinions in the post, but cannot be certain whether they are in disagreement with any previous posts.\\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \caption{The categories of the variable \textbf{H6. Conviction}.}
  \label{tab:H6}
  \centering
  \begin{tabular}{@{}p{2.5cm}@{\hspace{2mm}}p{15cm}@{}}
    \toprule
    \textbf{Variable} & \textbf{Definition and Explanation}\\
    \midrule
    \textbf{H6. Conviction} &
    The Level of Conviction shown by the arguments in the post (related to ``Rhetorical'' and ``Concession'' in RST).\\
    \midrule
    \textbf{Category} & \textbf{Definition and Explanation}\\
    \midrule
    \emph{Neutral} &
    The post does not show any opinion. This includes typical posts for seeking information or advice. However, it does not include posts that change or question existing guidelines.\\
    \emph{Doubtful} &
    The post expresses some doubts about a guideline or some opinions in the previous posts (e.g., through some mild questions) but does not explicitly give an opinion ``for'' or ``against''.\\
    \emph{Suggestive} &
    The post has at least one opinion, and all opinions are expressed in an uncertain way, with words such as ``perhaps'', ``possibly'', etc.\\
    \emph{Affirmative} &
    The post has at least one affirmative opinion, with words such as ``must'', ``should'', ``cannot be'', ``should never'', etc.\\
    \emph{Unclear} &
    The coder cannot determine if the post contains any opinion, e.g., the English expression in the post is difficult to understand.\\
    \bottomrule
  \end{tabular}
\end{table*}

==> sections/OldTexFiles/textanalytics.tex <==
\section{Text Analysis and Visualization}% (1-1.5 pages)}
\label{sec:TextAnalytics}
% Menna

%Considering that the \EDIT{subsets $D_{20190313}$ and $D_{Swansea2020}$} are text data sets collected in a visualization context, we are inspired to apply text analysis and visualization to it. 
While manually coding posts and categories is a practical necessity as well as scientifically rewarding, automatic text analysis and visualization may reveal patterns and insight that close reading cannot.  
In many ways, we can consider automatic text analysis and visualization as a form of ``open coding'' performed through computation. 
We argue that as long as human analysts are involved in comparative analysis and knowledge discovery, objective text analysis and visualization can complement the traditional GT methodology. 

In this section, we applied text analysis and visualization to a subset,~\dtextanalysis{}, of 84 posts from \dataset{} to illustrate our approach and report on findings (\textbf{Q2}). In particular, we applied a text analysis as a tool to understand: (1) possible hierarchies of topics, (2) commonly debated concepts and how they relate to guidelines, (3) relationships among key concepts about guidelines, and (4) the study of dynamics between participants in the discourse based on sentiment relations in the underlying text collection.

%\EDIT{The subset contains all the posts until 13/03/2019, named subset $D_{20190313}$.}

\begin{figure}%[hb!]
    \centering
    \includegraphics[width=\columnwidth]{figures/TextAnalysis/lexical_episodes_annotated.pdf}
    \caption{ The Lexical Episode Plot~\cite{Gold15} depicts the evolution of the discussion over time. It automatically detects \textit{compact chains of $n$-grams} and highlights them beside the complete text as an \textit{overview}. We can interactively zoom-in to the interesting text areas for \textit{close-reading}. Detailed figures can be found on the appendix C.}
    \label{fig:LEP}
    \vspace{-4mm}
\end{figure}

\subsection{\textbf{Tools}}
The analysis of forum discussions is an active area of research~\cite{Liu2018} with the goals of capturing the dynamics of topics, participants, as well as the linguistic quality of the posts and utterances. Such a type of text data bears the characteristics of verbatim text, i.e., it is based on social interactions, with a rapid creation cycle and evolution. 
%In contrast to highly-edited text from books and articles, this type of text brings along the challenge of being more noisy and heterogeneous~\cite{Hautli-Janisz2017a}. 

In this section, we used the \textit{VisArgue platform}~\cite{El-Assady2017c} a linguistic visualization framework specialized in analyzing conversational text, such as in political debates and forums. 
%That platform integrates a multi-step linguistic pipeline with state-of-the-art statistical processing and machine learning, providing a wide set of visual designs as perspective on the given input data. For instance, for the analysis of forum data, the \textit{ThreadReconstructor}~\cite{El-Assady2018b} visualization offers a technique for untangling threaded discussions; \textit{sequential pattern mining}~\cite{DBLP:conf/vissym/JentnerEGK17} techniques can reveal patterns in parallel conversational corpora; to reveal the dynamics between conversation participants, \textit{ConToVi}~\cite{EGA+16a} applies topic modeling, as well as micro-linguistic feature detection, highlighting the argumentation and language use styles of speakers.  
% R1-13: Some of the numeric analysis and manipulation of the data is either inadequately described, poorly justified or questionable. For example, "From the data set D20190313, we extracted 84 posts". How, which, Why?
%
%For each thread, the XML structure of $D_{20190313}$ consists of an initial question and subsequent replies.
From the 84 selected posts, we removed any URLs, images, and stop-words and eliminated the posts that contain only administrative messages.
% I wouldn't mention social conversations unless you can carefully define them
% and social conversations.
% R1-14: "Removing images and stop words seems arbitrary if undertaking GT. This is data. Why remove certain types of data? One could argue that graphics are important sources of data in discourse about visualization. Removing them and focusing on text only seems unnecessary and will certainly bias findings."
We then employed several techniques to reveal the contextual relationships among these posts.
%
%The main goal of our visual text analysis is to address the challenge of categorizing visualization guidelines.  
%Based on statistical analysis, we deduced that the 11 current categories of guidelines of VisGuides are not ideal.
% R1-15: "In places assumptions that influence the work are not made explicit. For the text analysis, it seems that ""the statistical analysis"" is basically counting the numbers of posts in each category and deciding that they are uneven? If yes, then the term ""statistical analysis"" is overstating it. If so, then I don't understand how Q3 emerges from the GT - this seems to be a straightforward count of posts?"
%\EDIT{The current categories at VisGuides represent the initial set up, based only individual main topics that visualization guidelines might cover, but they do not cover possible relationship across topics, for example, or the influence of a topic to another.
%We applied a data-driven text analysis as an statistical tool understand (1) possible hierarchies of topics, (2) common debated concepts and how do they relate to guidelines, and (3) the relationship among key extracted concepts on the discussed guidelines.}
%% reviewers' comment 
% R1-16: "By "a more informed categorization" do you mean a more even one? Because reality isn't even. The existing categories are likely to be indicative of something - most posts in a public forum about design guidelines used by people who are willing to engage in public debates abut knowledge categorise their contributions as "Visual Design" from the current closed set. That's useful or informative. Or maybe it tells us that popular post topics attract posts. Or that unpopular post topics don't. This requires more thought."
%We further use visual text analytics to study the dynamics between participants in the discourse based on sentiment relations in the underlying text collection.   
\subsection{Analysis Methods}

\paragraph{\textbf{Lexical Episode Plots:}}
We first used \textit{Lexical Episode Plots}~\cite{Gold15} to analyze the evolution of the discussions. This technique extracts densely occurring lexical chains, as visualized in \autoref{fig:LEP}.  Objects are placed on a zoomable canvas to enable a smooth transition between close- and distant-reading.  Threads are placed in chronological order (from top to bottom) and abstracted with gray blocks for distant-reading. 
Each of the blocks fades into its respective text when zoomed-in to enable close-reading. 
On the left-hand side, the extracted \textit{episodes} are layed out. 
These are $n$-grams that occur more densely than expected if we assume a uniform distribution of words.
Every occurrence of an \textit{episode} is marked by a horizontal line on its respective bar, as well as a colored bar at the word's position in the thread.
From \autoref{fig:LEP}, a human coder can observe a number of keywords (e.g., \textit{colormap}, \textit{spatial}, and \textit{treemap}) that may be considered potentially as topics. 
It also shows a potential co-occurrence relationship between keywords \textit{color\_map} and \textit{perceptual}. Appendix C includes more detailed visualizations from which we can observe other potential topics (e.g., \textit{interaction}, \textit{parallel coordinates}, \textit{design}, \textit{3D}, \textit{bubble}, \textit{dimension}, etc.).  

% 1. Is time goes from top (past) to bottom (recent)?

% 2. What do the width and height of the grey block encode?

% 3. keywords on the right seems to show mainly uni-gram. Am I correct that they are selected by ranking. What is the window for computing such ranking?

% For example, there are "visualise" "visualization" "visualization" in three places. Does this suggest that whole time axis is divided to 3 or more sections for compute the ranking?

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/TextAnalysis/network-w-inset.pdf}
    \caption{ The Named Entity Graph~\cite{El-Assady2017} depicts the relationship between the most \textit{relevant} entity pairs in a corpus, i.e., entities occurring more often together than an expected threshold. In this graph instance, the node ``color'' is very prominent, as the use of rainbow colormaps has been extensively discussed in the underlying text. Detailed figures can be found on the appendix C.}
    \label{fig:NEREx-small}
    \vspace{-4mm}
\end{figure}

\begin{figure}%[hb!]
    \centering
    \includegraphics[width=\columnwidth]{figures/TextAnalysis/topic_tree-w-inset.pdf}
    \caption{ The Topic Tree~\cite{el2018visual} \textit{groups all semantically-related utterances} (as leaf nodes) in a hierarchical tree structure with inner-nodes constituting topics and sub-topics. The \textit{outer border} of the tree depicts the \textit{top-descriptors} of each topic branch and the \textit{uncertainty of the respective utterance assignment} to that topic. Detailed figures can be found on the appendix C.}
    \label{fig:topics-small}
    \vspace{-4mm}
\end{figure}

\paragraph{\textbf{Named Entity Graph:}}
The second technique we used is the \textit{Named Entity Graph}~\cite{El-Assady2017}, as shown in Figures \ref{fig:NEREx-small} and \ref{fig:NEREx}. This visualization approach is based on named-entity recognition~\cite{manning2014stanford}, dividing descriptive words into ten categories. It considers entities to be related, if they occur within the same sentence in a window of a given size (here: five).  The number of times two entities occur together in a corpus determines their edge weight.  Using a force-directed layout, entities (nodes) are placed on a canvas, connected by directed edges (showing the order in which the entity pair appears in the text).  Nodes are additionally color-coded to show their category, e.g., purple nodes for content keywords, blue nodes for organizations, orange nodes for person names, and green and red nodes for positive and negative sentiment respectively.  The size of each node encodes the number of times this entity appears in the text.  In the example shown in \autoref{fig:NEREx-small}, the above-mentioned discussion on \textit{colormaps} is again prominent in the lower-right corner of the graph, accompanied by the keywords \textit{rainbow}, \textit{easier}, and \textit{harmful}.  In the upper-right corner, conversational keywords are connected with the entity ``\textit{Swansea University}'', referring to the %data collected in the 
assignment described as part of the Swansea data collection.


\paragraph{\textbf{Incremental Hierarchical Topic Modelling:}}
The third technique we applied is \textit{Incremental Hierarchical Topic Modeling}~\cite{El-Assady2018ProgressiveFramework} to extract the \textit{Topic Tree} shown in \autoref{fig:topics-small}. This technique groups all posts (as leaf nodes) in a hierarchical tree structures (with all inner nodes considered topics and sub-topics). On the outer edge of the tree, the \textit{topic descriptors} for the level-1 branches are shown. Using a technique called \textit{topic backbone}~\cite{El-Assady2018ProgressiveFramework} the topic tree can be primed towards expected clusters.  If found, these are shown as the outermost keywords, e.g., \textit{Color}, \textit{Temporal Visualization}, etc. Other clusters found in the topic tree include topics on \textit{Interaction} and \textit{Virtual Reality}, as well as a large group on a discourse on \textit{health} data.  In addition, smaller topics such as one on commercial visualization software (keyword: \textit{tableau}) have been extracted as thematically separable from the rest of the topics in the tree.

% Hence, to analyze a corpus of forum conversations on visualization guidelines, we employed different techniques such as Named-Entity Recognition~\cite{manning2014stanford}, Topic Modeling~\cite{El-Assady2018ProgressiveFramework}, and Lexical Chaining~\cite{Gold15}. 

\subsection{Findings}
Using text analysis as an additional means of open coding has complemented the manual GT processes reported in Section \ref{sec:VisGuides}, while text visualization has enabled us to connect the keywords and relationships identified by algorithms with the insights obtained from close reading. From text visualization, we made the following observations addressing the research question \textbf{Q2}.
%
\begin{itemize}[noitemsep, leftmargin=*]
  \item We identified a number of keywords correlating to specific visual representations, such as, \emph{parallel coordinates} or \emph{treemap}. This suggests a \textbf{potential hierarchy of guidelines} with the most important contexts organized as topics with subtopics. It could be desirable to define guideline topics or sub-topics based on such contexts.

  \item Some keywords, such as, \emph{color}, \emph{shape}, \emph{space}, \emph{time}, and \emph{perception} are generic to many posts, which indicates that \textbf{some guideline topics are more generic}. Such keywords can provide guidance on another aspect of categorizing visualization guidelines on overarching themes. At the same time such analysis will be able to show topic clusters.
  
  \item The relationships among various keywords (as shown in Figs. \ref{fig:LEP}, \ref{fig:NEREx}, and \ref{fig:topics}) are prominent in seeking and offering advice with or without using guidelines, and relationships between different concepts should ideally be featured in a \textbf{taxonomy of visualization guidelines}. This finding echoes a similar conclusion based on the language analysis of guideline expressions as found by Kandogan et al.~\cite{kandogan2016grounded}.
  
  \item The \textbf{keywords and relationships} identified from VisGuides data sets are supposed to continue evolving in the coming months and years. They are useful for prompting users to consider other keywords and relationships that may be featured in different contexts, e.g., research, education, and professional practice, and under different conditions.
 For example, guidelines such as ``Tufte’s Data-Ink ratio'', ``carefully use visual embellishment'', and ``Don’t Replicate the Real World in VR'' might not appear immediately related but they may have a point in common that needs further research and discussion.
  
 % \item In addition to the individual posts and threads, more information may be extracted from conversational fragments, cross-talks, and common places among threads. Therefore, further text analysis and visualization, e.g., using the \textit{VisArgue platform}, may enable us to make new discoveries. \ben{are there any findings about that? If not, it has to be removed from our motivation in the beginning of this section.
 

% R1-10: ""The finding that ""posing a critical question or offering a critical comment is not common"" is much less controversial than the previous findings. Many of the assertions are not made with evidence or conviction. In S5, why is it ""desirable to define topics or sub-topics based on such contexts"" (idioms) Where in the analysis in S5 is anything detected that might support the notion that ""The keywords and relationships identified from VisGuides data sets will continue to evolve in the coming years""?
\end{itemize}

% Based on our visual text analysis we could gain a better insight into the discourse. Since the utilized methods are data-driven and objective, we could determine potential categorizations of the discussion content that were not supported by a top-down solution. However, 

% Furthermore, connected keywords (as shown in \autoref{fig:NEREx} and \autoref{fig:topics}) suggest that the guideline categorization has to consider the relationships between two or more concepts (topics, or keywords), posing a challenge to a categorization scheme or taxonomy. 

%  Firstly, from n-grams to keywords (informing the selection of categories). Secondary, the keywords may depend on other facts, such as time and users. Thirdly, keywords are connected (Fig. 4), suggesting that guideline categorization has to consider the relationships between two or more concepts (topics, or keywords), posing a challenge to a categorization scheme or taxonomy. (ii) the visualization also makes observation of clusters easy, especially the Swansea student cluster (providing a link to the next section.)

% \noindent Difficulties with categorization of visualization guidelines.\\
% The current categories.\\
% Using text analysis to study the discourse\\

% In terms of Fig. 3(a),
% For Fig. 3(b),

% 4. how are the topics around the ring determined?

% 5. Are they related to the keywords in Fig. 3(a) in some way?

% For Fig. 4. What are the coding scheme:

% Node color:
% Node side:
% Note glyph:
% Note outline: ... 


% Both the Lexical Episode Plot~\cite{Gold15} and the Topic Tree~\cite{el2018visual} reveal the \textit{contextual relationships} of different discussion utterances.

% \textcolor{red}{I need two sentences here on the data source and preparation.. }
% We have analyzed xx topic conversations \textcolor{red}{I have 84 but you might have filtered a few more} from VisGuides since its beginning in September 27, 2017 until March 13, 2019. 
% The common structure consists of an initial question and subsequent replies. 
% The question and replies can contain text and supporting images, URLs, and videos.
% We have pre-processed the URLs, images, and stop-words from the text and eliminated the threads that did not provide any insight into the use of guidelines, i.e: welcome messages, and general information of the forum.
% After the pre-processing, we proceed with the text analysis using VisArgue.


